Adversarial Neural Networks for Error Correcting Codes

Error correcting codes are a fundamental component in modern day communication systems, demanding extremely high throughput, ultra-reliability and low latency. Recent approaches using machine learning (ML) models as the decoders offer both improved performance and great adaptability to unknown environments, where traditional decoders struggle. We introduce a general framework to further boost the performance and applicability of ML models. We propose to combine ML decoders with a competing discriminator network that tries to distinguish between codewords and noisy words, and, hence, guides the decoding models to recover transmitted codewords. Our framework is game-theoretic, motivated by generative adversarial networks (GANs), with the decoder and discriminator competing in a zero-sum game. The decoder learns to simultaneously decode and generate codewords while the discriminator learns to tell the differences between decoded outputs and codewords. Thus, the decoder is able to decode noisy received signals into codewords, increasing the probability of successful decoding. We show a strong connection of our framework with the optimal maximum likelihood decoder by proving that this decoder defines a Nash equilibrium point of our game. Hence, training to equilibrium has a good possibility of achieving the optimal maximum likelihood performance. Moreover, our framework does not require training labels, which are typically unavailable during communications, and, thus, seemingly can be trained online and adapt to channel dynamics. To demonstrate the performance of our framework, we combine it with the very recent neural decoders and show improved performance compared to the original models and traditional decoding algorithms on various codes.

==> ECC_Globecom 2021_submit/algorithm1.tex <==
\section{Proposed model}
\label{sec:alg}

Motivated by the generative adversarial network (GAN), our proposed model combines deep unfolding neural network model with a discriminator that distinguishes between valid codewords and outputs of the unfolding model. The decoder and discriminator competes in game: the decoder tries to fool the discriminator in thinking that its outputs are valid codes, or, maximize the classification error; on the other hand, the discriminator is a classification model that tries to tell which inputs are original valid codes and which are generated by the decoder. Effectively, the two models improve each other at the same time as the better decoder or discriminator gives better feedback to the other of how to improve.

==> ECC_Globecom 2021_submit/algorithm2.tex <==
\section{Proposed model}
\label{sec:alg}

Motivated by the recent advances in GANs, we propose to combine deep unfolding neural network models with a discriminator that distinguishes between codewords following the uniform distribution and decoded outputs of the unfolding network.
The decoder and discriminator compete in a zero-sum game: the decoder tries to fool the discriminator into thinking that its outputs are codewords, i.e., maximizing the classification error; on the other hand, the discriminator is a classification model that tries to tell which input sequences are original codewords and which are generated by the decoder.
Effectively, the two models improve at the same time as the better decoder or discriminator gives better feedback to the other about how to improve to better compete.

\subsection{Model architecture}
\begin{figure}[!h]
	\centering
	\vspace{-0.1in}
	\includegraphics[width=1\linewidth]{fig/proposed_model_l.pdf}
	\vspace{-0.1in}
	\caption{Proposed model architecture where decoder and discriminator networks compete and improve together as both are trained till equilibrium.}
	\label{fig:proposed_model}
\end{figure}

The proposed model is described in Figure~\ref{fig:proposed_model}.
The BP unfolded decoder network $G$ takes the received noisy signal from the channel and produces the decoded output $\hat \x$. The discriminator network $D$ is a classification model and aims at discriminating between codewords $\x$ and decoded outputs $\hat \x$ from the decoder.
The cost function $f(G,D)$ evaluates how well the discriminator network performs.
Thus, the goal of decoder is the opposite with that of the discriminator, which is maximizing the loss function.

Let $\mathcal{U}$ denote the uniform distribution generating random codewords and $\mathcal{P}_G$ the resulting distribution of the decoder's outputs. We overload the notations $\mathcal{U}$ and $\mathcal{P}_G$ to denote both the distribution and probability mass function.
We use the following common loss function in generative adversarial networks:
\begin{align}
	\label{eq:f_gd}
	f(G,D) = \mathbb{E}_{\x \sim \mathcal{U}} [\log D(\x)] + \mathbb{E}_{\y \sim \mathcal{P}_G} [\log(1 - D(\y))].
\end{align}
This function measures how well the discriminator classifies codewords from decoded outputs.
In other words, the discriminator tries to maximize this function while the decoder aims at minimizing it.
Hence, the optimization problem is to find $G^*$ and $D^*$ that solve the following min-max problem:
\begin{align}
	\label{eq:opt_problem}
	\min_{G}\max_{D} \mathbb{E}_{\x \sim \mathcal{U}} [\log D(\x)] + \mathbb{E}_{\y \sim \mathcal{P}_G} [\log (1 - D(\y))],
\end{align}
where $G$ is the BP unfolded network with parameters $w_{i,v}, w_{i,e,e'}$ and $w_{2L+1,v,e'}$, and $D$ is a classification model within some class of models.
As we will show later, with different classes of classification models, we can prove various results regarding the equilibrium between decoder and discriminator with respect to the min-max game in Eq.~(\ref{eq:opt_problem}).

\subsection{Theoretical results}

\subsubsection{Approaching optimal maximum likelihood performance}
\label{subsec:approach_ml}

We first prove that our model has a strong connection with the optimal ML decoder that is computationally intractable in practice due to its hardness.
We show that the ML decoder along with a discriminator trained with the ML decoder is in fact an equilibrium of our min-max game defined in Eq.~(\ref{eq:opt_problem}).
Let $G_{ML}$ represent the optimal ML decoder and $D_{ML}$ be defined as follows:
\begin{align}
	\label{eq:dml_prob}
	D_{ML} = \argmax_{D} \mathbb{E}_{\x \sim \mathcal{U}} [\log D(\x)] + \mathbb{E}_{\y \sim \pgml} [\log (1 - D(\y))].
\end{align}
Note that $D$ is in the class of all possible classification models.

From \cite{goodfellow2014generative}, we have the following lemma characterizing $\dml$ based on $\gml$.
\begin{lemma}
	\label{lem:dml_opt}
	Let $D$ be from the class of all classification models.
	The solution $\dml$ for problem (\ref{eq:dml_prob}) with respect to fixing $G$ to be $\gml$, i.e., having distribution $\pgml$, is
	\begin{align}
		\dml(x) = \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}, \forall \x \in \mathbb{C}.
	\end{align}
\end{lemma}

We establish the following theorem showing that $\gml$ and $\dml$ form an equilibrium of our min-max problem in (\ref{eq:opt_problem}).
\begin{theorem}
	\label{theo:ml_equi}
	The optimal ML decoder $\gml$ and the corresponding discriminator $\dml$ form an equilibrium for our min-max problem in (\ref{eq:opt_problem}).
	Specifically, we have
	\begin{align}
%		\label{eq:ml_equi}
		\max_{D} f(\gml, D) \leq f(\gml, \dml) \leq \min_{G} f(G, \dml), \nonumber
	\end{align}
	where $f(G,D)$ is defined in Eq.~(\ref{eq:f_gd}) and $G$ is from the class of all unfolded BP networks with different weight parameters $w_{i,v}, w_{i,e,e'}$ and $w_{2L+1,v,e'}$ as defined in Eq.~(\ref{eq:m_vc}) and Eq.~(\ref{eq:o_v}).
\end{theorem}
\begin{proof}$ $
	
	The first inequality $\max_{D} f(\gml, D) \leq f(\gml, \dml)$ follows immediately from the definition of $\dml$ in Lemma~\ref{lem:dml_opt} that $\dml$ is the optimal classification model with respect to the optimal ML decoder $\gml$.
	
	To prove the second inequality $f(\gml, \dml) \leq \min_{G} f(G, \dml)$, consider the function $f(G, \dml)$.
	We have
	\begin{align}
		\label{eq:14}
		f(G, \dml) &= \mathbb{E}_{\x \sim \mathcal{U}} [\log \dml(\x)] + \mathbb{E}_{\y \sim \mathcal{P}_G} [\log (1 - \dml(\y))] \nonumber \\
		& = \mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\ 
		& \qquad + \mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log (1 - \frac{\mathcal{U}(\y)}{\mathcal{U}(\y) + \pgml(\y)})\right] \nonumber \\
		& = \mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
		& \qquad + \mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right].
	\end{align}

	Regarding the optimization problem of $f(G, \dml)$ over $G$, the first term in Eq.~(\ref{eq:14}) is fixed for all $G$ and we can focus on the second term with $\y \sim \mathcal{P}_G$.
	For any $\y \not\in \mathbb{C}$ and $\pgml(\y) \neq 0$, $\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}$ achieves its maximum value of $0$ since $\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)} \leq 0$.
	Therefore, to minimize $f(G,\dml)$, we can narrow our consideration to decoders that produce only codewords.
	Furthermore, due to the symmetry of linear block codes, $\pgml$ is the uniform distribution over codewords.
	Thus, for any decoder $G$ that only produces codewords, we have
	\begin{align}
		\label{eq:15}
		& \mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right] \nonumber \\ 
		& = \mathbb{E}_{\y \sim \pgml} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right] = \log \frac{1}{2}.
	\end{align}
	
	Taking the minimization over all BP unfolding networks $G$ in Eq.~(\ref{eq:14}) and incorporating Eq.~(\ref{eq:15}) into Eq.~(\ref{eq:14}), we obtain
	\begin{align}
		\min_{G} f(G, \dml) & = \min_{G} \Big(\mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
		& \text{ \ \ } + \mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right] \Big) \nonumber \\
		& \geq \mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
		& \text{ \ \ } + \min_{G} \left(\mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right]\right) \nonumber \\
		& = \mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
		& \text{ \ \ } + \mathbb{E}_{\y \sim \pgml} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right] \nonumber \\
		& = f(\gml, \dml).
	\end{align}
	That completes the proof of the second inequality and the theorem.
%	We rewrite the term of interest as follows:
%	\begin{align}
%		\mathbb{E}_{y \sim \mathcal{P}_G} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right] = \mathbb{E}_{x \sim \mathcal{U}, r \sim \mathcal{G}(0, \sigma^2)} \left[ \log \frac{\pgml(G(x+r))}{\mathcal{U}(G(x+r)) + \pgml(G(x+r))} \right],
%	\end{align}
%	where $r \sim \mathcal{G}(0, \sigma^2)$ is the random noise following the Gaussian distribution with mean $0$ and variance $\sigma^2$.
\end{proof}

The equilibrium point corresponding to the optimal ML decoder suggests that if we train our BP unfolding network till convergence to an equilibrium, we can possibly achieve the optimal ML decoding performance.
This possibility is high for the BP unfolding network since the original BP method is based on the Tanner graph of the code and the resulting BP solution also provides good approximations of the true likelihood over codewords in practice.

\subsubsection{Model simplification and preserving BP fixed points}
\label{subsec:bp_fixed}

The number of weight parameters in the deep unfolding model is quite large, i.e., $O(L\cdot n + L\cdot E \cdot d_{max})$, where $L$ is the number of BP iterations, $E$ is the number of edges in the Tanner graph, and $d_{\max}$ denotes the maximum degree of any node.
We can improve the efficiency of our model by weight simplification.
%the following weight simplification scheme, motivated from practical observations, which also brings in another theoretical property. 
We simplify the weight parameters $w_{i,v}$ and $w_{i,e,e'}$ of layer $i$ in the unfolding network into a single weight parameter $w_i$ and reduce the total number of trainable weights to $L$.
This stems from our experimental observations that most of the parameters in the same layer have similar values after training.
Intuitively, this simplification helps reduce the computation in both training and running the model. 

The BP method on factor graphs has been studied extensively in the literature \cite{yedidia2001characterization,yedidia2003understanding,kuck2020belief,satorras2020neural} and shown to have interesting properties.
Among those properties, an important one is the correspondence of BP fixed points to solutions of the Bethe free energy defined on the factor graph \cite{yedidia2001characterization,yedidia2003understanding}.
The solutions minimizing the Bethe free energy provide a lower-bound for the factor graph's partition function, which is useful for inferences on the graph.
A set of messages is a fixed point of BP if they remain the same values after updates in Eq.~(\ref{eq:m_vc_bp}) and Eq.~(\ref{eq:m_cv_bp}).
We can derive a variant of our model that preserves all the fixed points of BP method in a straightforward manner.
Specifically, let $\bar{x}_{i,e=(v,c)}$ be the updated message from variable node $v$ to check node $c$ for the original BP method in Eq.~(\ref{eq:m_vc_bp}).
The activation function in odd layer $i$ is modified to
\begin{align}
	\label{eq:m_vc_variant}
	x_{i, e = (v,c)} = & (\bar{x}_{i,e} - \bar{x}_{i-1,e}) \Big[w_{i,v}l_v \nonumber \\
	& + \sum_{e' = (c',v), c' \neq c} w_{i,e,e'}x_{i-1, e'}\Big] + \bar{x}_{i-1,e}.
\end{align}
The activation function on the even layers are the same as in the original model, i.e., Eq.~(\ref{eq:m_cv}).

%More importantly, it leads to a critical theoretical result that the BP unfolding network preserves all the fixed point solutions of the original BP method. Thus, our simplified model inherits all the interesting theoretical properties of BP method including its correspondence of fixed points to solutions of Bethe approximation \cite{yedidia2001characterization,yedidia2003understanding}, which provides a lower-bound for the factor graph's partition function in our case.

We obtain the following result regarding the relation between BP fixed points and our simplified deep unfolding model.

\begin{proposition}
	The simple variant of the deep unfolding network with activation function in Eq.~(\ref{eq:m_vc_variant}) preserves all the fixed points of the original belief propagation (BP) method.
\end{proposition}
\begin{proof}
	The proof is evident from the definition of fixed points.
	The set of $\bar{x}_{i,e=(v,c)}$ and $\bar{x}_{i,(e = (c,v))}$ is a fixed point of BP if $\bar{x}_{i,e=(v,c)} = \bar{x}_{i-1,e=(v,c)}$ and $\bar{x}_{i,(e = (c,v))} = \bar{x}_{i-1,(e = (c,v))}$ for all $(c,v)$ and $(v,c)$.
	Plugging these conditions into the activation functions of our model variant in Eq.~(\ref{eq:m_cv}) and Eq.~(\ref{eq:m_vc_variant}), we also obtain the same conditions for fixed points that $x_{i,e=(v,c)} = x_{i-1,e=(v,c)} = \bar{x}_{i-1,e=(v,c)}$ and $x_{i,(e = (c,v))} = x_{i-1,(e = (c,v))} = \bar{x}_{i-1,(e = (c,v))}$.
	Hence, any fixed point of BP is also a fixed point of our model.
\end{proof}

\subsection{Online training for channel dynamics adaptation}

Compared to the deep unfolding model by itself, an advantageous characteristic of our game model is that it only requires received noisy signals from the channel and codewords which can be generated uniformly using the generator matrix of the code.
This property makes our model amenable to online training and effectively adapting to channel dynamics.
Specifically, we can collect batches of received signals and generate random batches of codewords to continually train our model on the fly.
This is in contrast to the deep unfolding model alone, which requires both the channel noisy signals and the true transmitted codewords to train it.

%\kwang{We will add details about GAN specifically designed for our model.}

%Summary of technical results (12/14/2020):
%\begin{itemize}
%    \item For weight simplification scheme that uses 1 single trainable weight value in each layer, we can show that this simplified model preserves fixed point solutions of the original belief propagation (BP) algorithm. Since the original BP's fixed point solution solves Bethe approximation, our model also has this property and can potentially do better theoretically thanks to trainable weight values. Also, because of solving Bethe approximation, showing the correspondence to ML optimal criteria is hard.
%    \item Our combination with GAN actually drives the deep unfolding network towards ML optimal criteria by enforcing a necessary condition of being ML optimal, that is the average of model output distribution must be uniform. Imagine each noisy input gives a distribution over valid codewords and if we average out all the distributions for all possible noisy inputs, ML optimal criteria gives us a uniform distribution. This property is provided by GAN property at equilibrium.
%\end{itemize}

==> ECC_Globecom 2021_submit/algorithm3.tex <==
\section{Proposed Model}
\label{sec:alg}

Motivated by the recent advances in GANs, we propose to combine deep unfolding neural network models with a discriminator that distinguishes between codewords following the uniform distribution and decoded outputs of the unfolding network.
The decoder and discriminator compete in a zero-sum game: the decoder tries to fool the discriminator into thinking that its outputs are codewords, i.e., maximizing the classification error; on the other hand, the discriminator is a classification model that tries to tell which input sequences are original codewords and which are generated by the decoder.
Effectively, the two models improve at the same time as the better decoder or discriminator gives better feedback to the other about how to improve to better compete.

\subsection{Model Architecture}
\begin{figure}[!t]
	\centering
	\vspace{-0.15in}
	\includegraphics[width=0.9\linewidth]{fig/proposed_model_l.pdf}
%	\vspace{-0.1in}
	\caption{Proposed model architecture where decoder and discriminator networks compete and improve together as both are trained till equilibrium.}
	\vspace{-0.15in}
	\label{fig:proposed_model}
\end{figure}

The proposed model is described in Figure~\ref{fig:proposed_model}.
The BP unfolded decoder network $G$ takes the received noisy signal from the channel and produces the decoded output $\hat \x$. The discriminator network $D$ is a classification model and aims at discriminating between codewords $\x$ and decoded outputs $\hat \x$ from the decoder.
The cost function $f(G,D)$ evaluates how well the discriminator network performs.
Thus, the goal of decoder is the opposite with that of the discriminator, which is maximizing the loss function.

Let $\mathcal{U}$ denote the uniform distribution generating random codewords and $\mathcal{P}_G$ the resulting distribution of the decoder's outputs.
Here, we slightly abuse notation and use $\mathcal{U}$ and $\mathcal{P}_G$ to denote both a distribution and a probability mass function.
We use the following common loss function in generative adversarial networks:
\begin{align}
	\label{eq:f_gd}
  f(G,D) = \mathbb{E}_{x \sim \mathcal{U}} [\log D(x)] + \mathbb{E}_{y \sim \mathcal{P}_G} [\log(1 - D(y))].
	% f(G,D) = \mathbb{E}_{\x \sim \mathcal{U}} [\log D(\x)] + \mathbb{E}_{\y \sim \mathcal{P}_G} [\log(1 - D(\y))].
\end{align}
This function measures how well the discriminator classifies codewords from decoded outputs.
In other words, the discriminator tries to maximize this function while the decoder aims at minimizing it.
Hence, the optimization problem is to find $G^*$ and $D^*$ that solve the following min-max problem:
\begin{align}
	\label{eq:opt_problem}
  \min_{G}\max_{D} \mathbb{E}_{x \sim \mathcal{U}} [\log D(x)] + \mathbb{E}_{y \sim \mathcal{P}_G} [\log (1 - D(y))],
	% \min_{G}\max_{D} \mathbb{E}_{\x \sim \mathcal{U}} [\log D(\x)] + \mathbb{E}_{\y \sim \mathcal{P}_G} [\log (1 - D(\y))],
\end{align}
where $G$ is the BP unfolded network with parameters $w_{i,v}, w_{i,e,e'}$ and $w_{2L+1,v,e'}$, and $D$ is a classification model within some class of models.
As we will show later, with different classes of classification models, we can prove various results regarding the equilibrium between decoder and discriminator with respect to the min-max game in Eq.~(\ref{eq:opt_problem}).

\subsection{Theoretical Results}

\subsubsection{Approaching optimal maximum likelihood performance}
\label{subsec:approach_ml}
We first prove that our model has a strong connection with the optimal ML decoder that is computationally intractable in practice due to its hardness.
We show that the ML decoder along with a discriminator trained with the ML decoder is in fact an equilibrium of our min-max game defined in Eq.~(\ref{eq:opt_problem}).
Let $G_{ML}$ represent the optimal ML decoder and $D_{ML}$ be defined as follows:
\begin{align}
	\label{eq:dml_prob}
  D_{ML} = \argmax_{D} \mathbb{E}_{x \sim \mathcal{U}} [\log D(x)] + \mathbb{E}_{y \sim \pgml} [\log (1 - D(y))].
	% D_{ML} = \argmax_{D} \mathbb{E}_{\x \sim \mathcal{U}} [\log D(\x)] + \mathbb{E}_{\y \sim \pgml} [\log (1 - D(\y))].
\end{align}
Note that $D$ is in the class of all possible classification models.

From \cite{goodfellow2014generative}, we have the following lemma characterizing $\dml$ based on $\gml$.
\begin{lemma}
	\label{lem:dml_opt}
	Let $D$ be from the class of all classification models.
	The solution $\dml$ for problem (\ref{eq:dml_prob}) with respect to fixing $G$ to be $\gml$, i.e., having distribution $\pgml$, is
	\begin{align}
    \dml(x) = \frac{\mathcal{U}(x)}{\mathcal{U}(x) + \pgml(x)}, ~ x \in C. \nonumber
		% \dml(x) = \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}, \forall \x \in \mathbb{C}. \nonumber
	\end{align}
\end{lemma}

We establish the following theorem showing that $\gml$ and $\dml$ form an equilibrium of our min-max problem in (\ref{eq:opt_problem}).
\begin{theorem}
	\label{theo:ml_equi}
	The optimal ML decoder $\gml$ and the corresponding discriminator $\dml$ form an equilibrium for our min-max problem in (\ref{eq:opt_problem}).
	Specifically, we have
	\begin{align}
%		\label{eq:ml_equi}
		\max_{D} f(\gml, D) \leq f(\gml, \dml) \leq \min_{G} f(G, \dml), \nonumber
	\end{align}
	where $f(G,D)$ is defined in Eq.~(\ref{eq:f_gd}) and $G$ is from the class of all unfolded BP networks with different weight parameters $w_{i,v}, w_{i,e,e'}$ and $w_{2L+1,v,e'}$ as defined in Eq.~(\ref{eq:m_vc}) and Eq.~(\ref{eq:o_v}).
\end{theorem}
\begin{proof}
	The first inequality $\max_{D} f(\gml, D) \leq f(\gml, \dml)$ follows immediately from the definition of $\dml$ in Lemma~\ref{lem:dml_opt} that $\dml$ is the optimal classification model with respect to the optimal ML decoder $\gml$.

	To prove the second inequality $f(\gml, \dml) \leq \min_{G} f(G, \dml)$, consider the function $f(G, \dml)$.
	We have
  \begin{align}
		\label{eq:14}
		f(G, \dml) &= \mathbb{E}_{x \sim \mathcal{U}} [\log \dml(x)] + \mathbb{E}_{y \sim \mathcal{P}_G} [\log (1 - \dml(y))] \nonumber \\
		& = \mathbb{E}_{x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(x)}{\mathcal{U}(x) + \pgml(x)}\right] \nonumber \\
		& \qquad + \mathbb{E}_{y \sim \mathcal{P}_G} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right].
	\end{align}
	% \begin{align}
	% 	\label{eq:14}
	% 	f(G, \dml) &= \mathbb{E}_{\x \sim \mathcal{U}} [\log \dml(\x)] + \mathbb{E}_{\y \sim \mathcal{P}_G} [\log (1 - \dml(\y))] \nonumber \\
	% 	% & = \mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
	% 	% & \qquad + \mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log (1 - \frac{\mathcal{U}(\y)}{\mathcal{U}(\y) + \pgml(\y)})\right] \nonumber \\
	% 	& = \mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
	% 	& \qquad + \mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right].
	% \end{align}

	Regarding the optimization problem of $f(G, \dml)$ over $G$, the first term in Eq.~(\ref{eq:14}) is fixed for all $G$ and we can focus on the second term with $y \sim \mathcal{P}_G$.
	For any $y \not\in C$ and $\pgml(y) \neq 0$, $\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}$ achieves its maximum value of $0$ since $\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)} \leq 0$.
	Therefore, to minimize $f(G,\dml)$, we can narrow our consideration to decoders that produce only codewords.
	Furthermore, due to the symmetry of linear block codes, $\pgml$ is the uniform distribution over codewords.
	Thus, for any decoder $G$ that only produces codewords, we have
	\begin{align}
		\label{eq:15}
    & \mathbb{E}_{y \sim \mathcal{P}_G} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right] \nonumber \\
		& = \mathbb{E}_{y \sim \pgml} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right] = \log \frac{1}{2}.
		% & \mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right] \nonumber \\
		% & = \mathbb{E}_{\y \sim \pgml} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right] = \log \frac{1}{2}.
	\end{align}

	Taking the minimization over all BP unfolding networks $G$ in Eq.~(\ref{eq:14}) and incorporating Eq.~(\ref{eq:15}) into Eq.~(\ref{eq:14}), we obtain
	\begin{align}
    \min_{G} f(G, \dml) & = \min_{G} \Big(\mathbb{E}_{x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(x)}{\mathcal{U}(x) + \pgml(x)}\right] \nonumber \\
		& \text{ \ \ } + \mathbb{E}_{y \sim \mathcal{P}_G} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right] \Big) \nonumber \\
		& = \mathbb{E}_{x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(x)}{\mathcal{U}(x) + \pgml(x)}\right] \nonumber \\
		& \text{ \ \ } + \min_{G} \left(\mathbb{E}_{y \sim \mathcal{P}_G} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right]\right) \nonumber \\
		& = \mathbb{E}_{x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(x)}{\mathcal{U}(x) + \pgml(x)}\right] \nonumber \\
		& \text{ \ \ } + \mathbb{E}_{y \sim \pgml} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right] \nonumber \\
		& = f(\gml, \dml).
		% \min_{G} f(G, \dml) & = \min_{G} \Big(\mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
		% & \text{ \ \ } + \mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right] \Big) \nonumber \\
		% & \geq \mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
		% & \text{ \ \ } + \min_{G} \left(\mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right]\right) \nonumber \\
		% & = \mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
		% & \text{ \ \ } + \mathbb{E}_{\y \sim \pgml} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right] \nonumber \\
		% & = f(\gml, \dml).
	\end{align}
	That completes the proof of the second inequality and the theorem.
%	We rewrite the term of interest as follows:
%	\begin{align}
%		\mathbb{E}_{y \sim \mathcal{P}_G} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right] = \mathbb{E}_{x \sim \mathcal{U}, r \sim \mathcal{G}(0, \sigma^2)} \left[ \log \frac{\pgml(G(x+r))}{\mathcal{U}(G(x+r)) + \pgml(G(x+r))} \right],
%	\end{align}
%	where $r \sim \mathcal{G}(0, \sigma^2)$ is the random noise following the Gaussian distribution with mean $0$ and variance $\sigma^2$.
\vspace{-0.05in}
\end{proof}

The equilibrium point corresponding to the optimal ML decoder suggests that if we train our BP unfolding network till convergence to an equilibrium, we can possibly achieve the optimal ML decoding performance.
This possibility is high for the BP unfolding network since the original BP method is based on the Tanner graph of the code and the resulting BP solution also provides good approximations of the true likelihood over codewords in practice.

\subsubsection{Preserving BP fixed points}
The BP method on factor graphs has been studied extensively in the literature \cite{yedidia2001characterization,yedidia2003understanding,kuck2020belief,satorras2020neural} and shown to have interesting properties.
Among those properties, an important one is the correspondence of BP fixed points to solutions of the Bethe free energy defined on the factor graph \cite{yedidia2001characterization,yedidia2003understanding}.
The solutions minimizing the Bethe free energy provide a lower-bound for the factor graph's partition function, which is useful for inferences on the graph.
A set of messages is a fixed point of BP if they remain the same values after updates in Eq.~(\ref{eq:m_vc_bp}) and Eq.~(\ref{eq:m_cv_bp}).
We can derive a variant of our model that preserves all the fixed points of BP method in a straightforward manner.
Specifically, let $\bar{x}_{i,e=(v,c)}$ be the updated message from variable node $v$ to check node $c$ for the original BP method in Eq.~(\ref{eq:m_vc_bp}).
The activation function in odd layer $i$ is modified to
\vspace{-0.05in}
\begin{align}
	\label{eq:m_vc_variant}
	x_{i, e = (v,c)} = & (\bar{x}_{i,e} - \bar{x}_{i-1,e}) \Big[w_{i,v}l_v \nonumber \\
	& + \sum_{e' = (c',v), c' \neq c} w_{i,e,e'}x_{i-1, e'}\Big] + \bar{x}_{i-1,e}.
\end{align}
The activation function on the even layers are the same as in the original model, i.e., Eq.~(\ref{eq:m_cv}).

%More importantly, it leads to a critical theoretical result that the BP unfolding network preserves all the fixed point solutions of the original BP method. Thus, our simplified model inherits all the interesting theoretical properties of BP method including its correspondence of fixed points to solutions of Bethe approximation \cite{yedidia2001characterization,yedidia2003understanding}, which provides a lower-bound for the factor graph's partition function in our case.

We obtain the following result regarding the relation between BP fixed points and our simplified deep unfolding model.

\begin{proposition}
	The simple variant of the deep unfolding network with activation function in Eq.~(\ref{eq:m_vc_variant}) preserves all the fixed points of the original belief propagation (BP) method.
\end{proposition}
\begin{proof}
	The proof is evident from the definition of fixed points.
	The set of $\bar{x}_{i,e=(v,c)}$ and $\bar{x}_{i,(e = (c,v))}$ is a fixed point of BP if $\bar{x}_{i,e=(v,c)} = \bar{x}_{i-1,e=(v,c)}$ and $\bar{x}_{i,(e = (c,v))} = \bar{x}_{i-1,(e = (c,v))}$ for all $(c,v)$ and $(v,c)$.
	Plugging these conditions into the activation functions of our model variant in Eq.~(\ref{eq:m_cv}) and Eq.~(\ref{eq:m_vc_variant}), we also obtain the same conditions for fixed points that $x_{i,e=(v,c)} = x_{i-1,e=(v,c)} = \bar{x}_{i-1,e=(v,c)}$ and $x_{i,(e = (c,v))} = x_{i-1,(e = (c,v))} = \bar{x}_{i-1,(e = (c,v))}$.
	Hence, any fixed point of BP is also a fixed point of our model.
\end{proof}
\subsubsection{Model simplification}
% \subsubsection{Model simplification and preserving BP fixed points}
\label{subsec:bp_fixed}

The number of weight parameters in the deep unfolding model is quite large, i.e., $O(L\cdot n + L\cdot E \cdot d_{max})$, where $L$ is the number of BP iterations, $E$ is the number of edges in the Tanner graph, and $d_{\max}$ denotes the maximum degree of any node.
We can improve the efficiency of our model by weight simplification.
%the following weight simplification scheme, motivated from practical observations, which also brings in another theoretical property.
We simplify the weight parameters $w_{i,v}$ and $w_{i,e,e'}$ of layer $i$ in the unfolding network into a single weight parameter $w_i$ and reduce the total number of trainable weights to $L$.
This stems from our experimental observations that most of the parameters in the same layer have similar values after training.
Intuitively, this simplification helps reduce the computation in both training and running.

\subsection{Online training for channel dynamics adaptation}

Compared to the deep unfolding model by itself, an advantageous characteristic of our game model is that it only requires received noisy signals from the channel and codewords which can be generated uniformly using the generator matrix of the code.
This property makes our model amenable to online training and effectively adapting to channel dynamics.
Specifically, we can collect batches of received signals and generate random batches of codewords to continually train our model on the fly.
This is in contrast to the deep unfolding model alone, which requires both the channel noisy signals and the true transmitted codewords to train it.

%\kwang{We will add details about GAN specifically designed for our model.}

%Summary of technical results (12/14/2020):
%\begin{itemize}
%    \item For weight simplification scheme that uses 1 single trainable weight value in each layer, we can show that this simplified model preserves fixed point solutions of the original belief propagation (BP) algorithm. Since the original BP's fixed point solution solves Bethe approximation, our model also has this property and can potentially do better theoretically thanks to trainable weight values. Also, because of solving Bethe approximation, showing the correspondence to ML optimal criteria is hard.
%    \item Our combination with GAN actually drives the deep unfolding network towards ML optimal criteria by enforcing a necessary condition of being ML optimal, that is the average of model output distribution must be uniform. Imagine each noisy input gives a distribution over valid codewords and if we average out all the distributions for all possible noisy inputs, ML optimal criteria gives us a uniform distribution. This property is provided by GAN property at equilibrium.
%\end{itemize}


==> ECC_Globecom 2021_submit/algorithm4.tex <==
\section{Proposed Framework}
\label{sec:alg}

Motivated by the recent advances in generative adversarial networks (GANs), we propose to combine a decoder model, e.g., unfolded BP network model, with a discriminator that distinguishes between codewords following the uniform distribution and decoded outputs of the decoder.
The decoder and discriminator compete in a zero-sum game: the decoder tries to fool the discriminator into thinking that its outputs are codewords, i.e., maximizing the classification error; on the other hand, the discriminator is a classification model that tries to tell which input sequences are original codewords and which are generated by the decoder.
Effectively, the two models improve simultaneously as the better decoder or discriminator gives better feedback to the other about how to improve to compete better.

\subsection{Architecture} \label{subsec:model}
\begin{figure}[!t]
	\centering
%	\vspace{-0.15in}
	\includegraphics[width=\linewidth]{fig/proposed_model_l.pdf}
%	\vspace{-0.1in}
	\caption{Proposed framework with decoder and discriminator networks competing and improving each other.}
%	\vspace{-0.15in}
	\label{fig:proposed_model}
\end{figure}

The proposed framework is described in Figure~\ref{fig:proposed_model}.
The decoder network $G$ takes the noisy signal from the channel and produces the decoded output $\hat x$, e.g., $o_v$ in Eq.~\ref{eq:o_v}. The discriminator network $D$ is a classification model and aims at discriminating between codewords $x$ and decoded outputs $\hat x$ from the decoder.
The function $f(G,D)$ evaluates how well the discriminator network performs.
Thus, the decoder's goal is the opposite of the discriminator's, minimizing $f(G,D)$.

Let $\mathcal{U}$ denote the uniform distribution generating random codewords and $\mathcal{P}_G$ the resulting distribution of the decoder's outputs.
Here, we slightly abuse notation and use $\mathcal{U}$ and $\mathcal{P}_G$ to denote both a distribution and a probability mass function.
We use the following common objective function in GANs:
\begin{align}
	\label{eq:f_gd}
  f(G,D) = \mathbb{E}_{x \sim \mathcal{U}} [\log D(x)] + \mathbb{E}_{y \sim \mathcal{P}_G} [\log(1 - D(y))].
	% f(G,D) = \mathbb{E}_{\x \sim \mathcal{U}} [\log D(\x)] + \mathbb{E}_{\y \sim \mathcal{P}_G} [\log(1 - D(\y))].
\end{align}
This function measures how well the discriminator classifies codewords from decoded outputs.
In other words, the discriminator tries to maximize this function while the decoder aims at minimizing it.
Hence, the optimization problem is to find $G^*$ and $D^*$ that solve the following min-max problem:
\begin{align}
	\label{eq:opt_problem}
  \min_{G}\max_{D} \mathbb{E}_{x \sim \mathcal{U}} [\log D(x)] + \mathbb{E}_{y \sim \mathcal{P}_G} [\log (1 - D(y))],
	% \min_{G}\max_{D} \mathbb{E}_{\x \sim \mathcal{U}} [\log D(\x)] + \mathbb{E}_{\y \sim \mathcal{P}_G} [\log (1 - D(\y))],
\end{align}
where $G$ is the decoder network with parameters $w_{i,v}, w_{i,e,e'}$ and $w_{2L+1,v,e'}$, and $D$ is a classification model within some class of models.
As we will show later, with different classes of classification models, we can prove various results regarding the equilibrium between decoder and discriminator with respect to the min-max game in Eq.~(\ref{eq:opt_problem}).


\subsection{Theoretical Properties}

\subsubsection{Approaching the Optimal Maximum Likelihood Performance}
\label{subsec:approach_ml}
We first prove that our model has a strong connection with the optimal maximum likelihood decoder, which is computationally intractable in practice due to its hardness.
We show that the maximum likelihood decoder along with a discriminator network trained with this decoder is, in fact, an Nash's equilibrium of our min-max game defined in Eq.~(\ref{eq:opt_problem}).
Let $G_{ML}$ represent the optimal maximum likelihood decoder and $D_{ML}$ be defined as follows:
\begin{align}
	\label{eq:dml_prob}
  D_{ML} = \argmax_{D} \mathbb{E}_{x \sim \mathcal{U}} [\log D(x)] + \mathbb{E}_{y \sim \pgml} [\log (1 - D(y))].
	% D_{ML} = \argmax_{D} \mathbb{E}_{\x \sim \mathcal{U}} [\log D(\x)] + \mathbb{E}_{\y \sim \pgml} [\log (1 - D(\y))].
\end{align}
Note that $D$ is in the class of all possible classification models.

From \cite{goodfellow2014generative}, we have the following lemma characterizing $\dml$ based on $\gml$.
\begin{lemma}
	\label{lem:dml_opt}
	Let $D$ be from the class of all classification models.
	The solution $\dml$ for problem (\ref{eq:dml_prob}) with respect to fixing $G$ to be $\gml$, i.e., having distribution $\pgml$, is
	\begin{align}
    \dml(x) = \frac{\mathcal{U}(x)}{\mathcal{U}(x) + \pgml(x)}, ~ x \in C. \nonumber
		% \dml(x) = \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}, \forall \x \in \mathbb{C}. \nonumber
	\end{align}
\end{lemma}

Based on the above lemma, we establish the following theorem showing that $\gml$ and $\dml$ form an equilibrium of our min-max problem in (\ref{eq:opt_problem}).
\begin{theorem}
	\label{theo:ml_equi}
	The optimal maximum likelihood decoder $\gml$ and the corresponding discriminator $\dml$ form an equilibrium for our min-max problem in (\ref{eq:opt_problem}).
	Specifically, we have
	\begin{align}
%		\label{eq:ml_equi}
		\max_{D} f(\gml, D) \leq f(\gml, \dml) \leq \min_{G} f(G, \dml), \nonumber
	\end{align}
	where $f(G,D)$ is defined in Eq.~(\ref{eq:f_gd}) and $G$ is from the class of all decoder networks with different weight parameters, i.e.,  $w_{i,v}, w_{i,e,e'}$ and $w_{2L+1,v,e'}$ as defined in Eq.~(\ref{eq:m_vc}) and Eq.~(\ref{eq:o_v}).
\end{theorem}
\begin{proof}
	The first inequality $\max_{D} f(\gml, D) \leq f(\gml, \dml)$ follows immediately from the definition of $\dml$ in Lemma~\ref{lem:dml_opt} that $\dml$ is the optimal classification model with respect to the optimal maximum likelihood decoder $\gml$.

	To prove the second inequality $f(\gml, \dml) \leq \min_{G} f(G, \dml)$, consider the function $f(G, \dml)$.
	We have
  \begin{align}
		\label{eq:14}
		f(G, &\dml) \nonumber \\
		&= \mathbb{E}_{x \sim \mathcal{U}} [\log \dml(x)] + \mathbb{E}_{y \sim \mathcal{P}_G} [\log (1 - \dml(y))] \nonumber \\
		& = \mathbb{E}_{x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(x)}{\mathcal{U}(x) + \pgml(x)}\right] \nonumber \\
		& \qquad + \mathbb{E}_{y \sim \mathcal{P}_G} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right].
	\end{align}
	% \begin{align}
	% 	\label{eq:14}
	% 	f(G, \dml) &= \mathbb{E}_{\x \sim \mathcal{U}} [\log \dml(\x)] + \mathbb{E}_{\y \sim \mathcal{P}_G} [\log (1 - \dml(\y))] \nonumber \\
	% 	% & = \mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
	% 	% & \qquad + \mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log (1 - \frac{\mathcal{U}(\y)}{\mathcal{U}(\y) + \pgml(\y)})\right] \nonumber \\
	% 	& = \mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
	% 	& \qquad + \mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right].
	% \end{align}
	Regarding the optimization problem of $f(G, \dml)$ over $G$, the first term in Eq.~(\ref{eq:14}) is fixed for all $G$ and we can focus on the second term with $y \sim \mathcal{P}_G$.
	For any $y \not\in C$ and $\pgml(y) \neq 0$, $\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}$ achieves its maximum value of $0$ since $\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)} \leq 0$.
	Therefore, to minimize $f(G,\dml)$, we can narrow our consideration to decoders that produce only codewords.
	Furthermore, due to the symmetry of linear block codes, $\pgml$ is the uniform distribution over codewords.
	Thus, for any decoder $G$ that only produces codewords, we have
	\begin{align}
		\label{eq:15}
    & \mathbb{E}_{y \sim \mathcal{P}_G} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right] \nonumber \\
		& = \mathbb{E}_{y \sim \pgml} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right] = \log \frac{1}{2}.
		% & \mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right] \nonumber \\
		% & = \mathbb{E}_{\y \sim \pgml} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right] = \log \frac{1}{2}.
	\end{align}

	Taking the minimization over all decoder networks $G$ in Eq.~(\ref{eq:14}) and incorporating Eq.~(\ref{eq:15}) into Eq.~(\ref{eq:14}), we obtain
	\begin{align}
    \min_{G} f(G, \dml) & = \min_{G} \Big(\mathbb{E}_{x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(x)}{\mathcal{U}(x) + \pgml(x)}\right] \nonumber \\
		& \text{ \ \ } + \mathbb{E}_{y \sim \mathcal{P}_G} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right] \Big) \nonumber \\
		& = \mathbb{E}_{x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(x)}{\mathcal{U}(x) + \pgml(x)}\right] \nonumber \\
		& \text{ \ \ } + \min_{G} \left(\mathbb{E}_{y \sim \mathcal{P}_G} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right]\right) \nonumber \\
		& = \mathbb{E}_{x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(x)}{\mathcal{U}(x) + \pgml(x)}\right] \nonumber \\
		& \text{ \ \ } + \mathbb{E}_{y \sim \pgml} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right] \nonumber \\
		& = f(\gml, \dml),
		% \min_{G} f(G, \dml) & = \min_{G} \Big(\mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
		% & \text{ \ \ } + \mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right] \Big) \nonumber \\
		% & \geq \mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
		% & \text{ \ \ } + \min_{G} \left(\mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right]\right) \nonumber \\
		% & = \mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
		% & \text{ \ \ } + \mathbb{E}_{\y \sim \pgml} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right] \nonumber \\
		% & = f(\gml, \dml).
	\end{align}
	which completes the proof of the second inequality and the theorem.
%	We rewrite the term of interest as follows:
%	\begin{align}
%		\mathbb{E}_{y \sim \mathcal{P}_G} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right] = \mathbb{E}_{x \sim \mathcal{U}, r \sim \mathcal{G}(0, \sigma^2)} \left[ \log \frac{\pgml(G(x+r))}{\mathcal{U}(G(x+r)) + \pgml(G(x+r))} \right],
%	\end{align}
%	where $r \sim \mathcal{G}(0, \sigma^2)$ is the random noise following the Gaussian distribution with mean $0$ and variance $\sigma^2$.
%\vspace{-0.05in}
\end{proof}

The equilibrium point corresponding to the optimal maximum likelihood decoder suggests that if we train our framework till convergence to equilibrium, we can possibly achieve optimal maximum likelihood decoding performance.
This possibility is high for the unfolded BP network since its architecture is based on the Tanner graph that generates the code and, thus, the resulting network provides good approximations of the true likelihood over codewords.

\subsubsection{Preserving BP Fixed Points}
Specifically consider our example of unfolded BP network, we can say more about the properties of our framework that we can easily derive a variant to preserve all the \emph{fixed points} of the original BP algorithm.
We first define a fixed point of BP as a set of messages that remain the same values after updates in Eq.~(\ref{eq:m_vc_bp}) and Eq.~(\ref{eq:m_cv_bp}).
The BP method on factor graphs has been studied extensively in the literature \cite{yedidia2001characterization,yedidia2003understanding,kuck2020belief,satorras2020neural} and shown to have interesting properties.
Among those properties, an important one is the correspondence of BP fixed points to solutions of the Bethe free energy defined on a factor graph \cite{yedidia2001characterization,yedidia2003understanding}.
The solutions minimizing the Bethe free energy provide a lower-bound for the factor graph's partition function, which is useful for inferences on that graph.

We can derive a variant of our model that preserves all the fixed points of the BP method in a straightforward manner.
Specifically, let $\bar{x}_{i,e=(v,c)}$ be the updated message from variable node $v$ to check node $c$ for the original BP method in Eq.~(\ref{eq:m_vc_bp}).
The activation function in odd layer $i$ is modified to
\vspace{-0.05in}
\begin{align}
	\label{eq:m_vc_variant}
	x_{i, e = (v,c)} = & (\bar{x}_{i,e} - \bar{x}_{i-1,e}) \Big[w_{i,v}l_v \nonumber \\
	& + \sum_{e' = (c',v), c' \neq c} w_{i,e,e'}x_{i-1, e'}\Big] + \bar{x}_{i-1,e}.
\end{align}
The activation function on the even layers are the same as in the original model, i.e., Eq.~(\ref{eq:m_cv}).

%More importantly, it leads to a critical theoretical result that the BP unfolding network preserves all the fixed point solutions of the original BP method. Thus, our simplified model inherits all the interesting theoretical properties of BP method including its correspondence of fixed points to solutions of Bethe approximation \cite{yedidia2001characterization,yedidia2003understanding}, which provides a lower-bound for the factor graph's partition function in our case.

We obtain the following result regarding the relation between BP fixed points and the variant of our model.
\begin{proposition}
	The simple variant of the deep unfolding network with activation function in Eq.~(\ref{eq:m_vc_variant}) preserves all the fixed points of the original belief propagation (BP) method.
\end{proposition}
\begin{proof}
	The proof is evident from the definition of fixed points.
	The set of $\bar{x}_{i,e=(v,c)}$ and $\bar{x}_{i,(e = (c,v))}$ is a fixed point of BP if $\bar{x}_{i,e=(v,c)} = \bar{x}_{i-1,e=(v,c)}$ and $\bar{x}_{i,(e = (c,v))} = \bar{x}_{i-1,(e = (c,v))}$ for all $(c,v)$ and $(v,c)$.
	Plugging these conditions into the activation functions of our model variant in Eq.~(\ref{eq:m_cv}) and Eq.~(\ref{eq:m_vc_variant}), we also obtain the same conditions for fixed points that $x_{i,e=(v,c)} = x_{i-1,e=(v,c)} = \bar{x}_{i-1,e=(v,c)}$ and $x_{i,(e = (c,v))} = x_{i-1,(e = (c,v))} = \bar{x}_{i-1,(e = (c,v))}$.
	Hence, any fixed point of BP is also a fixed point of our model.
\end{proof}

\begin{figure*}[h]
	\centering
	\begin{subfigure}[b]{0.42\linewidth}
		\includegraphics[width=\linewidth]{fig/bch_15_11}
		\caption{BCH(15,11)}
	\end{subfigure}
	\begin{subfigure}[b]{0.42\linewidth}
		\includegraphics[width=\linewidth]{fig/bch_63_45}
		\caption{BCH(63,45)}
	\end{subfigure}
	%\includegraphics[width=0.7\linewidth]{fig/bch_15_11}
	\caption{Performance of different decoders on BCH codes.}
	%	\vspace{-0.15in}
	\label{fig:bch_fer}
\end{figure*}
\begin{figure*}[h]
	\centering
	\begin{subfigure}[b]{0.42\linewidth}
		\includegraphics[width=\linewidth]{fig/rs_15_11}
		\caption{RS(15,11)}
	\end{subfigure}
	\begin{subfigure}[b]{0.42\linewidth}
		\includegraphics[width=\linewidth]{fig/rs_31_27}
		\caption{RS(31,27)}
	\end{subfigure}
	%\includegraphics[width=0.7\linewidth]{fig/bch_15_11}
	\caption{Performance of different decoders on Reed-Solomon (RS) codes. SSID is an effective belief propagation method for RS.}
	%	\vspace{-0.15in}
	\label{fig:rs_fer}
\end{figure*}
\subsubsection{Unfolded BP Model Simplification}
% \subsubsection{Model simplification and preserving BP fixed points}
\label{subsec:bp_fixed}

The number of weight parameters in the deep unfolding model is quite large, i.e., $O(L\cdot n + L\cdot E \cdot d_{max})$, where $L$ is the number of BP iterations, $E$ is the number of edges in the Tanner graph, and $d_{\max}$ denotes the maximum degree of any node.
We can improve the efficiency of our model by weight simplification.
We simplify the weight parameters $w_{i,v}$ and $w_{i,e,e'}$ of layer $i$ in the unfolding network into a single weight parameter $w_i$ and reduce the total number of trainable weights to $L$.
This simplification stems from our experimental observations that most of the parameters in the same layer have similar values after training.
Intuitively, this simplification helps reduce the computation in both training and testing, while resulting in similar performance as the full weight model.

\subsection{Online Training for Channel Dynamics Adaptation}

Compared to the decoder network by itself, our model has a strong advantageous characteristic that it only requires received noisy signals from the channel and uniformly random codewords, which can be generated using the generator matrix of the code.
This property makes our model amenable to online training and effectively adapting to channel dynamics.
Specifically, we can collect batches of received signals and generate random batches of codewords to train our model on the fly continually.
This contrasts with a typical decoder network, e.g., the deep unfolding model, which requires both the received signals and their corresponding transmitted codewords to train it, restricting their applicability in scenarios where the transmitted signals are not available at the receiver side. That is the common case in wireless communication with changing environment. Moreover, even if channel changes can be detected quickly and transmitted data can be obtained, retraining the decoder network could take a long time. Differently, our framework involves no such delay of obtaining data and retraining the decoder network as we can train online.

%\kwang{We will add details about GAN specifically designed for our model.}

%Summary of technical results (12/14/2020):
%\begin{itemize}
%    \item For weight simplification scheme that uses 1 single trainable weight value in each layer, we can show that this simplified model preserves fixed point solutions of the original belief propagation (BP) algorithm. Since the original BP's fixed point solution solves Bethe approximation, our model also has this property and can potentially do better theoretically thanks to trainable weight values. Also, because of solving Bethe approximation, showing the correspondence to ML optimal criteria is hard.
%    \item Our combination with GAN actually drives the deep unfolding network towards ML optimal criteria by enforcing a necessary condition of being ML optimal, that is the average of model output distribution must be uniform. Imagine each noisy input gives a distribution over valid codewords and if we average out all the distributions for all possible noisy inputs, ML optimal criteria gives us a uniform distribution. This property is provided by GAN property at equilibrium.
%\end{itemize}


==> ECC_Globecom 2021_submit/conc.tex <==
\section{Conclusion}

We have proposed a game-theoretic framework that combines a decoder network with a discriminator, which compete in a zero-sum game.
The decoder tries to decode a received noisy signal from the communication channel while the discriminator tries to distinguish between codewords from the decoded words.
Both decoder and discriminator improve together to be better at their own tasks.
We show a strong connection between our model and the optimal maximum likelihood (ML) decoder as the ML decoder forms a Nash equilibrium in our game model.
Our experimental results confirm improved decoding performance compared to the recent deep learning models and the belief propagation method.

%\section*{Acknowledgements}
%This research was, in part, funded by the U.S. Government, Defense Advanced Research Projects Agency (DARPA) under contract no. HR00112090056.
%The views and conclusions contained in this document are those of the authors and should not be interpreted as representing the official policies, either expressed or implied, of the U.S. Government.

==> ECC_Globecom 2021_submit/conc2.tex <==
\section{Conclusion}

We have proposed a game-theoretic framework that combines a decoder network with a discriminator, which compete in a zero-sum game.
The decoder tries to decode a received noisy signal from the communication channel while the discriminator tries to distinguish between codewords from the decoded words.
Both decoder and discriminator improve together to be better at their own tasks.
We show a strong connection between our model and the optimal maximum likelihood decoder as this decoder forms a Nash's equilibrium in our game model.
Numerical results confirm improved decoding performance compared to recent ML models and traditional decoders.


==> ECC_Globecom 2021_submit/experiments1.tex <==
\section{Experiments}
We apply our model on decoding of BCH and Reed Solomon codes and compare the results to that of deep unfolding model.

\subsection{Setting}
We use the same deep unfolding model as in \cite{nachmani2018deep} that corresponds to 5 BP iterations and add a simple 2 layer fully connected layers discriminator with the hidden layer having size of 1024 and sigmoid activation function and output layer being a single neuron. We applied Adam optimizer with learning rate of 0.001 and batch size 64. 10000 codes are used for training and 100000 codes are for testing. We consider AWGN channel with various signal-to-noise (SNR) ratios.

\subsection{Results}
\begin{figure}[!h]
	\centering
	\includegraphics[width=0.7\linewidth]{fig/FER_15_11_log.png}
	\caption{FER results on BCH(15,11).}
	\label{fig:bch_15_11}
\end{figure}

==> ECC_Globecom 2021_submit/experiments2.tex <==
\section{Experiments}
\label{sec:exps}

We demonstrate the better decoding performance of our model in comparison with the original deep unfolding network and BP decoder on various codes.

\begin{figure}[!t]
	\centering
	\begin{subfigure}[b]{0.8\linewidth}
		\includegraphics[width=\linewidth]{fig/bch_15_11}
		\caption{BCH(15,11)}
	\end{subfigure}
	\begin{subfigure}[b]{0.8\linewidth}
		\includegraphics[width=\linewidth]{fig/bch_63_45}
		\caption{BCH(63,45)}
	\end{subfigure}
	%\includegraphics[width=0.7\linewidth]{fig/bch_15_11}
	\caption{Performance of different decoders on BCH code.}
	\label{fig:bch_fer}
\end{figure}
\begin{figure}[!t]
	\centering
	\begin{subfigure}[b]{0.8\linewidth}
		\includegraphics[width=\linewidth]{fig/rs_15_11}
		\caption{RS(15,11)}
	\end{subfigure}
	\begin{subfigure}[b]{0.8\linewidth}
		\includegraphics[width=\linewidth]{fig/rs_31_27}
		\caption{RS(31,27)}
	\end{subfigure}
	%\includegraphics[width=0.7\linewidth]{fig/bch_15_11}
	\caption{Performance of different decoders of Reed-Solomon codes (SSID is an effective belief propagation method for RS).}
	\label{fig:rs_fer}
\end{figure}

\subsection{Setting}
We tested on both BCH codes BCH(15,11), BCH(63,45), and Reed-Solomon codes RS(15,11), RS(31,27), with an AWGN channel and various signal-to-noise (SNR) ratios.
For BCH codes, we use the neural offset min-sum deep unfolding model, FNOMS, as in \cite{nachmani2018deep} that unfolds 5 BP iterations and adds a discriminator with two fully connected layers, each of size 1024 with sigmoid activation function, and a single neuron output layer.
For Reed-Solomon codes, the decoder network, namely DeepSSID, unfolds the Stochastic Shifting Based Iterative Decoding (SSID) model\cite{zhang2020iterative}.
We applied the Adam optimizer with learning rate of 0.001 for both decoder and discriminator training and batch size 64.
10000 and 100000 codewords are randomly drawn for training and testing, respectively.

%\kwang{Compare with the classic results of BCH codes with BP decoding. Provide the number of iterations for decoding for all schemes.}
%\kwang{As commented in the previous section, use truncation for the sum-product algorithm rather than the min-sum algorithm for a fair comparison with \cite{nachmani2018deep}. In general, the sum-product algorithm outperforms the min-sum algorithm.}

\subsection{Results}

We compare our model, denoted by \method, with the original deep unfolding model and BP method with 100 iterations.
The results are demonstrated in Figure~\ref{fig:bch_fer} for BCH codes and Figure~\ref{fig:rs_fer} for Reed-Solomon codes.
In both cases, the results show that \method{} achieves improved decoding performance compared to both previous deep unfolding networks and BP.
The improvement is approximately 0.5dB consistently across all signal-to-noise ratios and different codes.

Notably, the improvement of \method{} for shorter block length as in BCH(15,11) and RS(15,11) is more significant than for longer block length as in BCH(63,45) and RS(31,27).
This is possibly due to the fixed number of layers in the decoder network and suggests larger block codes may need more layers or deeper networks to perform well.

%Weight patterns when training in GAN model:
%\begin{figure}[!h]
%	\centering
%	\includegraphics[width=0.5\linewidth]{fig/gan_weight_pattern.png}
%	\caption{Weight patterns of deep unfolding network when training in GAN model.}
%	\label{fig:gan_weight_15_11}
%\end{figure}

==> ECC_Globecom 2021_submit/experiments3.tex <==
\section{Experiments}
\label{sec:exps}

We demonstrate the better decoding performance of our model in comparison with the original deep unfolding network and BP decoder on various codes.

\begin{figure*}[!t]
	\centering
	\begin{subfigure}[b]{0.41\linewidth}
		\includegraphics[width=\linewidth]{fig/bch_15_11}
		\caption{BCH(15,11)}
	\end{subfigure}
	\begin{subfigure}[b]{0.41\linewidth}
		\includegraphics[width=\linewidth]{fig/bch_63_45}
		\caption{BCH(63,45)}
	\end{subfigure}
	%\includegraphics[width=0.7\linewidth]{fig/bch_15_11}
	\caption{Performance of different decoders on BCH code.}
	\vspace{-0.15in}
	\label{fig:bch_fer}
\end{figure*}
\begin{figure*}[!t]
	\centering
	\begin{subfigure}[b]{0.41\linewidth}
		\includegraphics[width=\linewidth]{fig/rs_15_11}
		\caption{RS(15,11)}
	\end{subfigure}
	\begin{subfigure}[b]{0.41\linewidth}
		\includegraphics[width=\linewidth]{fig/rs_31_27}
		\caption{RS(31,27)}
	\end{subfigure}
	%\includegraphics[width=0.7\linewidth]{fig/bch_15_11}
	\caption{Performance of different decoders of Reed-Solomon codes (SSID is an effective belief propagation method for RS).}
	\vspace{-0.15in}
	\label{fig:rs_fer}
\end{figure*}
%\kwang{Can we use red, green, and blue? Also, how about using different line styles for different scheme in addition to different markers, which have already been applied, for b\&w print? These suggestion also can be applied to Fig. 4.}

\subsection{Setting}
We tested on both BCH codes BCH(15,11), BCH(63,45), and Reed-Solomon codes RS(15,11), RS(31,27), with an AWGN channel and various signal-to-noise (SNR) ratios.
For BCH codes, we use the neural offset min-sum deep unfolding model, FNOMS, as in \cite{nachmani2018deep} that unfolds 5 BP iterations and adds a discriminator with two fully connected layers, each of size 1024 with sigmoid activation function, and a single neuron output layer.
For Reed-Solomon codes, the decoder network, namely DeepSSID, unfolds the Stochastic Shifting Based Iterative Decoding (SSID) model\cite{zhang2020iterative}.
We applied the Adam optimizer with learning rate of 0.001 for both decoder and discriminator training and batch size 64.
10000 and 100000 codewords are randomly drawn for training and testing, respectively.

%\kwang{Compare with the classic results of BCH codes with BP decoding. Provide the number of iterations for decoding for all schemes.}
%\kwang{As commented in the previous section, use truncation for the sum-product algorithm rather than the min-sum algorithm for a fair comparison with \cite{nachmani2018deep}. In general, the sum-product algorithm outperforms the min-sum algorithm.}

\subsection{Results}

We compare our model, denoted by \method, with the original deep unfolding model and BP method with 100 iterations.
The results are demonstrated in Figure~\ref{fig:bch_fer} for BCH codes and Figure~\ref{fig:rs_fer} for Reed-Solomon codes.
In both cases, the results show that \method{} achieves improved decoding performance compared to both previous deep unfolding networks and BP.
The improvement is approximately 0.5dB consistently across all signal-to-noise ratios and different codes.

Notably, the improvement of \method{} for shorter block length as in BCH(15,11) and RS(15,11) is more significant than for longer block length as in BCH(63,45) and RS(31,27).
This is possibly due to the fixed number of layers in the decoder network and suggests larger block codes may need more layers or deeper networks to perform well.

%Weight patterns when training in GAN model:
%\begin{figure}[!h]
%	\centering
%	\includegraphics[width=0.5\linewidth]{fig/gan_weight_pattern.png}
%	\caption{Weight patterns of deep unfolding network when training in GAN model.}
%	\label{fig:gan_weight_15_11}
%\end{figure}


==> ECC_Globecom 2021_submit/experiments4.tex <==
%\kwang{Can we use red, green, and blue? Also, how about using different line styles for different scheme in addition to different markers, which have already been applied, for b\&w print? These suggestion also can be applied to Fig. 4.}

\section{Numerical Results}
\label{sec:exps}

We demonstrate the better decoding performance of our framework compared with the original decoder network and traditional decoding algorithms on various codes. Again, we consider the unfolded BP networks as the ML model in our experiments.

\subsection{Settings}
\textit{Error correcting codes and unfolded models:}
We run our experiments on two linear codes: BCH with BCH(15,11), BCH(63,45), and Reed-Solomon codes RS(15,11), RS(31,27), with an AWGN channel and various signal-to-noise ratios (SNRs).
For BCH codes, we use the neural offset min-sum deep unfolding model, FNOMS, as in \cite{nachmani2018deep} that unfolds 5 BP iterations and adds a discriminator with two fully connected layers, each of size 1024 with sigmoid activation function, and a single neuron output layer.
For Reed-Solomon codes, the decoder network, namely DeepSSID, unfolds 5 iterations of the Stochastic Shifting Based Iterative Decoding (SSID) model\cite{zhang2020iterative}. The same discriminator as above is also used for Reed-Solomon codes. Note that we deliberately use a very simple discriminator network here to  demonstrate the feasibility of deploying our framework in small devices with limited resources.

\textit{Train and test:}
We applied the Adam optimizer with a learning rate of 0.001 for training both decoder and discriminator and batch size of 64. 10000 and 100000 codewords are randomly drawn for training and testing, respectively. For our framework, we alternatively train decoder and discriminator as in a typical GAN training procedure.

\textit{Evaluation Metric:} We measure the performance of each method using Frame Error Rate (FER) as we focus on recovering the entire codeword or transmitted message.

%\kwang{Compare with the classic results of BCH codes with BP decoding. Provide the number of iterations for decoding for all schemes.}
%\kwang{As commented in the previous section, use truncation for the sum-product algorithm rather than the min-sum algorithm for a fair comparison with \cite{nachmani2018deep}. In general, the sum-product algorithm outperforms the min-sum algorithm.}

\subsection{Results}

We compare our framework, denoted by \method, with the neural unfolded BP model and the BP decoder with 100 iterations.
The results are demonstrated in Figure~\ref{fig:bch_fer} for BCH codes and Figure~\ref{fig:rs_fer} for Reed-Solomon codes.
In both cases, the results show that \method{} achieves improved decoding performance compared to both previous deep unfolding networks and BP.
The improvement is approximately 0.5 dB compared to the unfolding model by itself, and 1 dB in comparison to BP decoder, consistently across all frame error rates and different codes. On the contrary, unfolded BP networks only improve over BP decoder for large SNR values.

Notably, the improvement of \method{} for shorter block length as in BCH(15,11) and RS(15,11) is more significant than for longer block length as in BCH(63,45) and RS(31,27).
This is possibly due to the fixed number of layers in the decoder network and suggests larger block codes may need more layers or deeper networks to perform well. Nevertheless, both \method{} and the unfolded BP model only correspond to 5 BP iterations while the BP decoder needs 100 iterations and the performance are still much lower.
%Weight patterns when training in GAN model:
%\begin{figure}[!h]
%	\centering
%	\includegraphics[width=0.5\linewidth]{fig/gan_weight_pattern.png}
%	\caption{Weight patterns of deep unfolding network when training in GAN model.}
%	\label{fig:gan_weight_15_11}
%\end{figure}


==> ECC_Globecom 2021_submit/intro1.tex <==
\section{Introduction}

Deep unfolding \cite{hershey2014deep} combines the learning power of emerging deep neural networks (DNNs) with rigorous analytical understanding of model-based iterative algorithms in communications to address multiple challenges across various tasks, i.e., decoders for error correcting codes \cite{nachmani2018deep,lugosch2017neural,lugosch2018learning,zhang2020iterative}, symbol detection \cite{shlezinger2020deepsic,shlezinger2019viterbinet,samuel2019learning,he2018model}, channel precoding \cite{balatsoukas2019neural}. On one hand, deep unfolding removes assumptions of existing algorithms on channel condition and can deal with both linear and non-linear channels, while enjoying the optimality guarantees of well understood iterative algorithms thanks to having the same structure. On the other hand, deep unfolding can speed up the computation by reducing the number of iterations needed to achieve certain performance due to the impressive learnability of deep neural networks requiring only a few layers corresponding to a small number of iterations in existing iterative algorithms.

We propose to improve the performance of deep unfolding model by leveraging the same idea in  in the Generative Adversarial Networks (GANs) of having two models competing in a game and together improving their performances. In our case, we have the deep unfolding decoder learning to decode received noisy signal and we design a discriminator to distinguish between the decoded signal and valid codes. The goal of the decoder is both finding a sequence of symbols that is as close as possible to the transmitted one and fooling the discriminator to believe in that the generated sequence is a valid code. Hence, the decoder will be able to generate a valid code that is as close as possible to the transmitted code, boosting the probability of successful decoding. We illustrate our idea in Figure~\ref{fig:demo}. In the ideal case, the discriminator teaches the decoder to avoid invalid code regions and, thus, increases the probability of the decoder generating valid codes, including the correct codes with respect to the noisy received signal. Given that, error correcting codes has certain structure, the invalid region could be very large compared to valid region and, hence, the benefit of having this discriminator is significant.

\begin{figure}[!h]
	\centering
	\includegraphics[width=0.7\linewidth]{fig/demo.pdf}
	\caption{Benefit of having a discriminator to boost the probability of successful decoding.}
	\label{fig:demo}
\end{figure}

==> ECC_Globecom 2021_submit/intro2.tex <==
\section{Introduction}

Deep unfolding \cite{hershey2014deep} combines the learning power of emerging deep neural networks (DNNs) with rigorous analytical understanding of model-based iterative algorithms in communications to address multiple challenges across various tasks, e.g., decoders for error correcting codes \cite{nachmani2018deep,lugosch2017neural,lugosch2018learning,zhang2020iterative}, symbol detection \cite{shlezinger2020deepsic,shlezinger2019viterbinet,samuel2019learning,he2018model}, and MIMO precoding \cite{balatsoukas2019neural}.
On the one hand, deep unfolding removes assumptions of existing algorithms on channel condition and can deal with both linear and nonlinear channels, while enjoying the optimality guarantees of well understood iterative algorithms thanks to having the same structure \cite{yedidia2001characterization,kuck2020belief}.
On the other hand, deep unfolding can speed up the computation by reducing the number of iterations needed to achieve certain performance due to the impressive learnability of deep neural networks, requiring only a few layers corresponding to a small number of iterations in existing iterative algorithms.

%\begin{figure}[!h]
%	\centering
%	\includegraphics[width=0.8\linewidth]{fig/demo.pdf}
%	\caption{Benefit of having a discriminator to boost the probability of successful decoding.}
%	\label{fig:demo}
%\end{figure}

We propose to improve the performance of deep unfolding models by leveraging the same idea used in Generative Adversarial Networks (GANs) of having two models competing in a game and together improving their performances.
In our case, we have the deep unfolding decoder learning to decode a received (noisy) signal and design a discriminator to distinguish between codewords and the decoded words.
The goal of the decoder is both recovering a sequence that is as close as possible to the transmitted codeword and fooling the discriminator to believe in that the decoded sequence is an actual codeword.
Hence, the decoder will be able to recover a codeword that is as similar as possible to the transmitted one, boosting the probability of successful decoding.
% We illustrate our idea in Figure~\ref{fig:demo}. 
In the ideal case, the discriminator teaches the decoder to avoid non-codeword regions; thus, it increases the probability of the decoder recovering codewords, including the correct codeword with respect to the noisy received signals.
Given that an error correcting code has certain structure, the non-codeword region could be very large compared to codeword region and, hence, the benefit of having this discriminator is significant.

Our game-theoretical model combining a deep unfolding network and a discriminator enjoys multiple advantageous properties.
We first prove that the optimal maximum likelihood (ML) decoder of a code along with a custom trained discriminator form a Nash equilibrium of our game model (Subsection~\ref{subsec:approach_ml}).
This establishes a strong connection between our model and the optimal ML decoder; if we train the model till convergence (equilibrium), it has a good chance of approaching the optimal ML decoder.
Furthermore, we show that a simple variant of our model also preserves all the fixed points of the original belief propagation (BP) decoder (Subsection~\ref{subsec:bp_fixed}).
These fixed points correspond to solutions of minimizing the Bethe free energy \cite{yedidia2003understanding}, which is important for inference tasks on factor graphs.
We experimentally verify that our model leads to improved decoding performance on various error correcting codes when compared with the original deep unfolding model and the BP algorithm (Section~\ref{sec:exps}).

%\kwang{This reasoning is not clear as yet. $2^k$ codewords of a block code of length $n$ forms a $k$-dimensional subspace of the vector space of all the $n$-tuple over the field $GF(2)$; thus, for most good error correcting codes, the codeword space is much smaller the space of any other sequences. However, this does not necessarily mean that the benefit of having the discriminator is significant, because the existing decoders (either NN-optimized decoders or classic decoders) also aim to classify received sequences into a transmitted codeword or not by inherently avoiding invalid codewords region. We are digging into a question, ''How and how effectively the discriminator can play a role suppressing the invalid codewords region compared to the existing decoders' capabilities?'' Can theory behind GAN provide us more detailed guidance in designing NN-optimized decoding algorithms beyond our current understanding above? If so, how?}



==> ECC_Globecom 2021_submit/intro3.tex <==
\section{Introduction}
New data-intensive use cases (e.g., autonomous driving, high-precision industrial plants) demand high throughput and ultra-reliable and low latency communications for the fifth \cite{TS38.104} and subsequent generation networks. This demand requires iterative communication algorithms with a minimal number. However, little is theoretically known about optimal parameter tuning under strict iterative constraints and is usually established using heuristics via simulations or pessimistic bounds in practice \cite{Balatsoukas--Studer2019}.

%use cases and deployment requirements (e.g., eMBB and uRLLC in 5G NR) require information recovery with high throughput and/or very low latency for 5G \cite{TS38.104} and subsequent generation networks. This implies that iterative algorithms with a minimal number are desired. However, little is theoretically known about optimal parameter tuning under strict iterative constraints and is usually established using heuristics via simulations or pessimistic bounds in practice.

% Deep unfolding \cite{hershey2014deep} combines the learning power of emerging deep neural networks (DNNs) with rigorous analytical understanding of model-based iterative algorithms in communications to address multiple challenges across various tasks, e.g., decoders for error correcting codes \cite{nachmani2018deep,lugosch2017neural,lugosch2018learning,zhang2020iterative}, symbol detection \cite{shlezinger2020deepsic,shlezinger2019viterbinet,samuel2019learning,he2018model}, and MIMO precoding \cite{balatsoukas2019neural}.

Deep unfolding \cite{hershey2014deep} has been introduced as a promising approach to address these challenges across various tasks, e.g., decoders for error correcting codes \cite{nachmani2018deep,lugosch2017neural,lugosch2018learning,zhang2020iterative}, symbol detection \cite{shlezinger2020deepsic,shlezinger2019viterbinet,samuel2019learning,he2018model}, and MIMO precoding \cite{balatsoukas2019neural} by combining the learning power of emerging deep neural networks (DNNs) with rigorous analytical understanding of model-based  iterative algorithms in communications.
On the one hand, deep unfolding removes assumptions of existing algorithms on channel condition and can deal with both linear and nonlinear channels, while enjoying the optimality guarantees of well understood iterative algorithms thanks to having the same structure \cite{yedidia2001characterization,kuck2020belief}.
On the other hand, deep unfolding can speed up the computation by reducing the number of iterations needed to achieve certain performance due to the impressive learnability of deep neural networks, requiring only a few layers corresponding to a small number of iterations in existing iterative algorithms.

%\begin{figure}[!h]
%	\centering
%	\includegraphics[width=0.8\linewidth]{fig/demo.pdf}
%	\caption{Benefit of having a discriminator to boost the probability of successful decoding.}
%	\label{fig:demo}
%\end{figure}

We propose to improve the performance of deep unfolding models by leveraging the same idea used in Generative Adversarial Networks (GANs) of having two models competing in a game and together improving their performances.
In our case, we have the deep unfolding decoder learning to decode a received (noisy) signal and design a discriminator to distinguish between codewords and the decoded words.
The goal of the decoder is both recovering a sequence that is as close as possible to the transmitted codeword and fooling the discriminator to believe in that the decoded sequence is an actual codeword.
Hence, the decoder will be able to recover a codeword that is as similar as possible to the transmitted one, boosting the probability of successful decoding.
% We illustrate our idea in Figure~\ref{fig:demo}.
In the ideal case, the discriminator teaches the decoder to avoid non-codeword regions; thus, it increases the probability of the decoder recovering codewords, including the correct codeword with respect to the noisy received signals.
Given that an error correcting code has certain structure, the non-codeword region could be very large compared to codeword region and, hence, the benefit of having this discriminator is significant.

Our game-theoretical model combining a deep unfolding network and a discriminator enjoys multiple advantageous properties.
We first prove that the optimal maximum likelihood (ML) decoder of a code along with a custom trained discriminator form a Nash equilibrium of our game model (Subsection~\ref{subsec:approach_ml}).
This establishes a strong connection between our model and the optimal ML decoder; if we train the model till convergence (equilibrium), it has a good chance of approaching the optimal ML decoder.
Furthermore, we show that a simple variant of our model also preserves all the fixed points of the original belief propagation (BP) decoder (Subsection~\ref{subsec:bp_fixed}).
These fixed points correspond to solutions of minimizing the Bethe free energy \cite{yedidia2003understanding}, which is important for inference tasks on factor graphs.
We experimentally verify that our model leads to improved decoding performance on various error correcting codes when compared with the original deep unfolding model and the BP algorithm (Section~\ref{sec:exps}).


==> ECC_Globecom 2021_submit/intro4.tex <==
\section{Introduction}
New data-intensive use cases, e.g., autonomous driving, high-precision industrial plants, demand high throughput, ultra-reliable, and low latency communications for the fifth \cite{TS38.104} and subsequent generation networks. This demand requires communication algorithms to be performing and highly adaptive to any changes in the environment. For example, iterative error correcting codes' decoders need to operate with minimal number of iterations, while providing peak decoding performance at any time subject to channel variations. However, little is theoretically known about optimal parameter tuning under strict iterative constraints and it is usually established using heuristics via simulations or pessimistic bounds in practice \cite{Balatsoukas--Studer2019}, which limit the efficacy and applicability of those methods.

%use cases and deployment requirements (e.g., eMBB and uRLLC in 5G NR) require information recovery with high throughput and/or very low latency for 5G \cite{TS38.104} and subsequent generation networks. This implies that iterative algorithms with a minimal number are desired. However, little is theoretically known about optimal parameter tuning under strict iterative constraints and is usually established using heuristics via simulations or pessimistic bounds in practice.

% Deep unfolding \cite{hershey2014deep} combines the learning power of emerging deep neural networks (DNNs) with rigorous analytical understanding of model-based iterative algorithms in communications to address multiple challenges across various tasks, e.g., decoders for error correcting codes \cite{nachmani2018deep,lugosch2017neural,lugosch2018learning,zhang2020iterative}, symbol detection \cite{shlezinger2020deepsic,shlezinger2019viterbinet,samuel2019learning,he2018model}, and MIMO precoding \cite{balatsoukas2019neural}.

Machine learning approaches have been introduced recently as a promising candidate to address these challenges. As an exemplar, deep unfolding networks \cite{hershey2014deep} show great performance and channel adaptability across various tasks, such as decoders for error correcting codes \cite{nachmani2018deep,lugosch2017neural,lugosch2018learning,zhang2020iterative}, symbol detection \cite{shlezinger2020deepsic,shlezinger2019viterbinet,samuel2019learning,he2018model}, and MIMO precoding \cite{balatsoukas2019neural}, by combining the learning power of emerging deep neural networks (DNNs) with rigorous analytical understanding of model-based iterative algorithms in communications.
On one hand, deep unfolding removes the assumptions of existing algorithms on channel conditions and can deal with both linear and nonlinear channels, while retaining the interpretability of well understood iterative algorithms thanks to having the same structure \cite{yedidia2001characterization,kuck2020belief}.
On the other hand, deep unfolding can speed up computation by reducing the number of iterations required to achieve good performance due to the impressive learnability of DNNs, requiring only a few layers corresponding to a small number of iterations in existing iterative algorithms.
However, there is not a formal theoretical result about deep unfolding networks. All the properties of underlying algorithm are informally carried over to deep unfolding model due to structure sharing. 
%As a result, it might cause a large performance gap between deep unfolding networks and the optimal ML decoder.

We propose a framework to further boost the performance of ML models for the task of decoding error correcting codes by leveraging the same idea in generative adversarial networks (GANs) of having two models competing in a game and together improving their performances (Subsection~\ref{subsec:model}).
In our framework, we have an ML decoder learning to decode received (noisy) signals and design a discriminator to distinguish between (valid) codewords and decoder's outputs.
The goal of the decoder is 
%both recovering a sequence that is as close as possible to the transmitted codeword and 
to deceive the discriminator to believe in that its decoded sequences are an actual codewords.
% recover a codeword that is as similar as possible to the transmitted one, boosting the probability of successful decoding.
% We illustrate our idea in Figure~\ref{fig:demo}.
As the discriminator gets better in recognizing codewords, the decoder must learn to generate codeword-like sequences or to avoid non-codeword regions (typically significantly large). This can be seen as introducing an insightful constraint on the decoder's outputs in addition to existing ones on the decoder, e.g., structural constraints on deep unfolding networks. Thus, intuitively the decoder finds a codeword that is closest to the noisy signal with respect to some hidden metric defined by the discriminator, i.e., matching the distribution of true codewords.
%thus, this increases the probability of the decoder outputting codewords, including the transmitted one with respect to the received signal. 
%As a result, the decoder will be able to amplify the probability of successful decoding.
% Given that an error correcting code has certain structure, the non-codeword region could be very large compared to codeword region and, hence, the benefit of having this discriminator is significant.

Our game-theoretic framework, combining an ML decoder and a discriminator, enjoys multiple advantageous properties.
We first prove that the optimal maximum likelihood decoder of a code along with a custom trained discriminator form a Nash's equilibrium of our game model (Subsection~\ref{subsec:approach_ml}).
This establishes a strong connection between our model and the optimal maximum likelihood decoder: if we train the model till convergence (equilibrium), it has a good chance of approaching the optimal performance. Furthermore, applying our framework on the deep unfolding decoders \cite{lugosch2018learning,lugosch2017neural,zhang2020iterative}, that unfold several iterations of the belief propagation (BP) algorithm into a deep network, we show that a simple variant of our model also preserves all the fixed points of the original BP decoder (Subsection~\ref{subsec:bp_fixed}).
These fixed points correspond to solutions of minimizing the Bethe free energy \cite{yedidia2003understanding}, which is vital for inference tasks on factor graphs. More importantly, unlike existing models, our framework does not rely on training labels, i.e., transmitted signals, which are usually unavailable during communications, and thus has the capability of online training and adapts to any channel variations. We experimentally verify that our framework leads to improved decoding performance compared with the original deep unfolding models and the BP algorithms on various error correcting codes (Section~\ref{sec:exps}).

Throughout the paper, we use the unfolded BP networks \cite{lugosch2018learning,lugosch2017neural} (details in Section~\ref{sec:prelim}) as the demonstrating ML models in our framework for both the theory and experiments.


==> ECC_Globecom 2021_submit/preliminary1.tex <==
\section{Preliminaries}

Here we summarize the message passing belief propagation Sum-Product and Min-Sum algorithms along with their deep unfolding neural network models. 

\subsection{Belief propagation (BP) algorithms}

The belief propagation (BP) decoder for a linear code with some parity check matrix can be constructed from the Tanner graph of the parity check matrix. The Tanner graph contains check and variable nodes arranged as a bipartite graph, and edges between check and variable nodes, which represent messages passing between those nodes. Denote by $N$, the code block length (i.e., the number of variable nodes in the Tanner graph). A simple example is given in Figure~\ref{fig:bp}.(a) with $N = 3$ variable nodes. Each iteration in the BP decoder corresponds to one round of messaging passing between variable and check nodes. 
\begin{figure}[!h]
	\centering
	\includegraphics[width=0.7\linewidth]{fig/bp_illustrate.pdf}
	\vspace{-0.1in}
	\caption{Tanner graph and Trellis representation of a BP decoder.}
	\label{fig:bp}
\end{figure}
In iteration $i$, on the edge $e = (v,c)$ variable node $v$ passes the following message $x_{i, (v,c)}$ to the check node $c$:
\begin{align}
	x_{i, e = (v,c)} = l_v + \sum_{e' = (c',v), c' \neq c} x_{i-1, e'},
\end{align}
where $l_v$ is the log-likelihood ratio of the channel output corresponding to the $v$th codebit $C_v$:
\begin{align}
	l_v = \log\frac{\Pr(C_v = 1 | y_v)}{\Pr(C_v = 0 | y_v)}.
\end{align}

In the Sum-Product algorithm, the message $x_{i, (c,v)}$ from check node $c$ to variable node $v$ in iteration $i$ is computed as follows:
\begin{align}
	x_{i, e = (c,v)} = 2 \tanh^{-1}\left( \prod_{e' = (v',c), v' \neq v} \tanh \frac{x_{i,e'}}{2} \right).
\end{align}
However, this computation involves repeated multiplications and hyperbolic functions, which may lead to numerical problems in actual implementation. Thus the Min-Sum algorithm uses a ``min-sum'' approximation of the above message as follows:
\begin{align}
	x_{i, e = (c,v)} = \min_{e' = (v',c), v' \neq v} |x_{i,e'}| \prod_{e' = (v',c), v' \neq v} \sign(x_{i,e'}).
\end{align}

Suppose that BP decoder runs $L$ iterations, the final $v$th output is given by:
\begin{align}
	\label{eq:output}
	o_v = l_v + \sum_{e' = (c',v)} x_{L,e'}.
\end{align}

\subsection{Unfolding BP models}

The BP decoder has an equivalent Trellis representation that motivates the unfolding neural network architecture. An simple example is provided in Figure~\ref{fig:bp}.(b). Each BP iteration $i$ unfolds into 2 hidden layers $2\times i-1$ and $2\times i$ corresponding to 2 passes of message from variable to check nodes and, vice versus, from check to variable nodes. The number of nodes in each hidden layer is the same as the number of edges in the Tanner graph and, respectively, each node computes the message sent through each edge. Thus, there are $2\times L$ hidden layers in this Trellis representation in addition to an input and output layer. The input takes log-likelihood ratios of channel outputs and the output computes Eq.~\ref{eq:output}.

The unfolding neural network model share the exact same architecture as the Trellis representation and add trainable weights to the edges. Thus, in odd layer $i$, the computation at node $i, e = (v,c)$ perform the following operation:
\begin{align}
	x_{i, e = (v,c)} = \tanh \left(\frac{1}{2}\left (w_{i,v}l_v + \sum_{e' = (c',v), c' \neq c} w_{i,e,e'}x_{i-1, e'} \right) \right).
\end{align}
In even layer $i$, the computation at node $i, e = (v,c)$ is as follows:
\begin{align}
	x_{i, e = (c,v)} = 2 \tanh^{-1}\left( \prod_{e' = (v',c), v' \neq v} x_{i-1,e'} \right).
\end{align}
Node at the output layer performs:
\begin{align}
	o_v = \sigma \left(w_{2L + 1,v}l_v + \sum_{e' = (c',v)} w_{2L+1,v,e'} x_{2L,e'} \right ).
\end{align}

==> ECC_Globecom 2021_submit/preliminary2.tex <==
\section{Preliminaries}

In this section, we review the well known belief propagation (BP) method for error correcting codes and the deep neural network model that is constructed by deep unfolding this BP method.
Here we summarize the message passing belief propagation Sum-Product and Min-Sum algorithms along with their deep unfolding neural network models.

\textbf{Channel noise model.} We consider a common channel model where additive random noise follows a Gaussian distribution with mean $0$ and variance $\sigma^2$, i.e., $N(0, \sigma^2)$.
We follow the common assumption that transmitted codewords are uniformly selected at random from the set of all codewords.

\subsection{Belief propagation (BP) algorithms}

Given a linear error correcting code $\mathbb{C}$ of block-length $n$, characterized by a parity check matrix $\mathbf{H}$ of size $n \times (n-k)$, every codeword $\x \in \mathbb{C}$ satisfies $\mathbf{H}^T \x = \0$, where $\mathbf{H}^T$ denotes the transpose of $\mathbf{H}$ and $\0$ the vector of $n-k$ zeros.

The BP decoder for a linear code can be constructed from the Tanner graph of the parity check matrix.
The Tanner graph contains $n-k$ check nodes and $n$ variable nodes arranged as a bipartite graph with edges between check and variable nodes, which represent messages passing between these nodes.
If $\mathbf{H}_{vc} = 1$, there is an edge between variable node $v$ and check node $c$.
A simple example is given in Figure~\ref{fig:bp}(a) with $n = 3$ variable nodes and $(n-k) = 2$ check nodes.
The BP decoder consists of multiple iterations.
Each iteration corresponds to one round of messaging passing between variable and check nodes. 
\begin{figure}[!h]
	\centering
	\vspace{-0.1in}
	\includegraphics[width=\linewidth]{fig/bp_illustrate2.pdf}
	\caption{Tanner graph of a code and BP unfolding architecture.}
	\label{fig:bp}
\end{figure}
In iteration $i$, on edge $e = (v,c)$, the message $x_{i, (v,c)}$ passed from variable node $v$ to the check node $c$ is given by
\begin{align}
	\label{eq:m_vc_bp}
	x_{i, e = (v,c)} = l_v + \sum_{e' = (c',v), c' \neq c} x_{i-1, e'},
\end{align}
where $l_v$ is the log-likelihood ratio of the channel output corresponding to the $v$th codeword bit $C_v$.
Given random Gaussian noise, the log-likelihood ratio $l_v$ is
\begin{align}
	l_v = \log\frac{\Pr(C_v = 1 | y_v)}{\Pr(C_v = 0 | y_v)}.
\end{align}

In the Sum-Product algorithm, the message $x_{i, (c,v)}$ from check node $c$ to variable node $v$ in iteration $i$ is computed as
\begin{align}
	\label{eq:m_cv_bp}
	x_{i, e = (c,v)} = 2 \tanh^{-1}\left( \prod_{e' = (v',c), v' \neq v} \tanh \frac{x_{i,e'}}{2} \right).
\end{align}
For numerical stability, the messages going into a node in both Eq.~(\ref{eq:m_vc_bp}) and Eq.~(\ref{eq:m_cv_bp}) are normalized at every iteration and all the messages are also truncated within a fixed range.

Note that the computation in Eq.~(\ref{eq:m_cv_bp}) involves repeated multiplications and hyperbolic functions, which may lead to heavy computation and numerical problems in actual implementations.
Even with truncation of message values within a certain range, e.g., commonly $[-10, 10]$, we still observe numerical problems when running Sum-Product algorithm.

%\kwang{Truncate the messages from variable nodes to a check node into a specific range (e.g., -15.0 $\sim$ 15.0). It sets the size of the input messages in the check nodes to a level that does not cause numerical problems.}

The Min-Sum algorithm uses a ``min-sum'' approximation of the above message as follows:
\begin{align}
	x_{i, e = (c,v)} = \min_{e' = (v',c), v' \neq v} |x_{i,e'}| \prod_{e' = (v',c), v' \neq v} \sign(x_{i,e'}).
\end{align}

Suppose the BP decoder runs $L$ iterations. Then the $v$th output after final iteration is given by
\begin{align}
	\label{eq:output}
	o_v = l_v + \sum_{e' = (c',v)} x_{L,e'}.
\end{align}

\subsection{Unfolding BP models}

The BP decoder has an equivalent Trellis representation that motivates the unfolding neural network architecture.
A simple example is provided in Figure~\ref{fig:bp}(b).
Each BP iteration $i$ unfolds into 2 hidden layers, $2\times i-1$ and $2\times i$, corresponding to two passes of messages from variable to check nodes and from check to variable nodes.
The number of nodes in each hidden layer is the same as the number of edges in the Tanner graph and, respectively, each node computes the message sent through each edge.
Thus, there are $2\times L$ hidden layers in this Trellis representation in addition to an input and output layer.
The input takes log-likelihood ratios of channel received signals and the output computes Eq.~\ref{eq:output}.

The unfolding neural network model shares the same architecture as the Trellis representation and adds trainable weights to the edges.
In other words, in odd layer $i$, the computation at node $i, e = (v,c)$, performs the following operation (activation function):
\begin{align}
	\label{eq:m_vc}
	x_{i, e = (v,c)} = w_{i,v}l_v + \sum_{e' = (c',v), c' \neq c} w_{i,e,e'}x_{i-1, e'}.
\end{align}
Note that trainable weights $w_{i,v}$ and $w_{i,e,e'}$ are introduced in the computation.
These weights can be trained and address various challenging obstacles with the BP method: 1) reduce the large number of iterations needed in BP, leading to more efficiency; 2) improve decoding performance and possibly approach optimal ML criterion, thanks to the ability to possibly minimize the effects of short cycles known to cause difficulties for BP decoders.

In even layer $i$, the computation at node $i, e = (v,c)$ is similar to that in the regular BP algorithm:
\begin{align}
	\label{eq:m_cv}
	x_{i, e = (c,v)} = 2 \tanh^{-1}\left( \prod_{e' = (v',c), v' \neq v} \tanh \frac{x_{i-1,e'}}{2} \right).
\end{align}
For numerical stability, we also apply normalization and truncation of messages after every layer.

Nodes at the output layer perform
\begin{align}
	\label{eq:o_v}
	o_v = \sigma \left(w_{2L + 1,v}l_v + \sum_{e' = (c',v)} w_{2L+1,v,e'} x_{2L,e'} \right ),
\end{align}
where $\sigma(.)$ is the sigmoid function to obtain probability from the log-likelihood ratio representation.
Note that trainable weights $w_{2L + 1,v}$ and $w_{2L+1,v,e'}$ are also introduced here.

==> ECC_Globecom 2021_submit/preliminary3.tex <==
\section{Preliminaries}

In this section, we review the well known belief propagation (BP) method for error correcting codes and the deep neural network model that is constructed by deep unfolding this BP method.
Here we summarize the message passing belief propagation sum-product and min-sum algorithms along with their deep unfolding neural network models.

We consider the discrete-time additive white Gaussian noise (AWGN) channel model. In transmission time $i \in [1:n]$, the channel output is $Y_i = gX_i + Z_i$. where $g$ is the channel gain, $X_i \in \{ \pm 1\}$, $\{ Z_i \}$ is a AWGN ($\sigma^2$) process, independent of the channel input $X^n = x^n(m)$, $m \in [1:2^{k}]$, and $k$ is the message length.

% \textbf{Channel noise model.} We consider a common channel model where additive random noise follows a Gaussian distribution with mean $0$ and variance $\sigma^2$, i.e., $N(0, \sigma^2)$.
% We follow the common assumption that transmitted codewords are uniformly selected at random from the set of all codewords.

\subsection{Belief Propagation (BP) Algorithms}

Given a linear error correcting code $C$ of block-length $n$, characterized by a parity check matrix $H$ of size $n \times (n-k)$, every codeword $x \in C$ satisfies $H^T x = \0$, where $H^T$ denotes the transpose of $H$ and $0$ the vector of $n-k$ zeros.

% Given a linear error correcting code $\mathbb{C}$ of block-length $n$, characterized by a parity check matrix $\mathbf{H}$ of size $n \times (n-k)$, every codeword $\x \in \mathbb{C}$ satisfies $\mathbf{H}^T \x = \0$, where $\mathbf{H}^T$ denotes the transpose of $\mathbf{H}$ and $\0$ the vector of $n-k$ zeros.

The BP decoder for a linear code can be constructed from the Tanner graph of the parity check matrix.
The Tanner graph contains $n-k$ check nodes and $n$ variable nodes arranged as a bipartite graph with edges between check and variable nodes, which represent messages passing between these nodes.
If $H_{vc} = 1$, there is an edge between variable node $v$ and check node $c$.
% If $\mathbf{H}_{vc} = 1$, there is an edge between variable node $v$ and check node $c$.
A simple example is given in Figure~\ref{fig:bp}(a) with $n = 3$ variable nodes and $(n-k) = 2$ check nodes.
The BP decoder consists of multiple iterations.
Each iteration corresponds to one round of messaging passing between variable and check nodes.
\begin{figure}[!t]
	\centering
	\vspace{-0.1in}
	\includegraphics[width=\linewidth]{fig/bp_illustrate2.pdf}
	\caption{Tanner graph of a code and BP unfolding architecture.}
	\vspace{-0.15in}
	\label{fig:bp}
\end{figure}
In iteration $i$, on edge $e = (v,c)$, the message $x_{i, (v,c)}$ passed from variable node $v$ to the check node $c$ is given by
\begin{align}
	\label{eq:m_vc_bp}
	x_{i, e = (v,c)} = l_v + \sum_{e' = (c',v), c' \neq c} x_{i-1, e'},
\end{align}
where $l_v$ is the log-likelihood ratio of the channel output corresponding to the $v$th codeword bit $C_v$, i.e.,
% Given random Gaussian noise,
%The log-likelihood ratio $l_v$ is
\begin{align}
	l_v = \log\frac{\Pr(C_v = 1 | y_v)}{\Pr(C_v = 0 | y_v)}. \nonumber
\end{align}

In the sum-product algorithm, the message $x_{i, (c,v)}$ from check node $c$ to variable node $v$ in iteration $i$ is computed as
\begin{align}
	\label{eq:m_cv_bp}
	x_{i, e = (c,v)} = 2 \tanh^{-1}\Big( \prod_{e' = (v',c), v' \neq v} \tanh \frac{x_{i,e'}}{2} \Big).
\end{align}
For numerical stability, the messages going into a node in both Eq.~(\ref{eq:m_vc_bp}) and Eq.~(\ref{eq:m_cv_bp}) are normalized at every iteration and all the messages are also truncated within a fixed range.

Note that the computation in Eq.~(\ref{eq:m_cv_bp}) involves repeated multiplications and hyperbolic functions, which may lead to numerical problems in actual implementations. Even with truncation of message values within a certain range, e.g., commonly $[-10, 10]$, we still observe numerical problems when running the sum-product algorithm.
% Thus, we consider the Min-Sum algorithm in this paper.

% Note that the computation in Eq.~(\ref{eq:m_cv_bp}) involves repeated multiplications and hyperbolic functions, which may lead to heavy computation and numerical problems in actual implementations.
% Even with truncation of message values within a certain range, e.g., commonly $[-10, 10]$, we still observe numerical problems when running Sum-Product algorithm.

%\kwang{Truncate the messages from variable nodes to a check node into a specific range (e.g., -15.0 $\sim$ 15.0). It sets the size of the input messages in the check nodes to a level that does not cause numerical problems.}

The min-sum algorithm uses a ``min-sum'' approximation of the above message as follows:
\begin{align}
	x_{i, e = (c,v)} = \min_{e' = (v',c), v' \neq v} |x_{i,e'}| \prod_{e' = (v',c), v' \neq v} \sign(x_{i,e'}). \nonumber
\end{align}
Suppose the BP decoder runs $L$ iterations. Then the $v$th output after final iteration is given by
\begin{align}
	\label{eq:output}
	o_v = l_v + \sum_{e' = (c',v)} x_{L,e'}.
\end{align}

\subsection{Unfolding BP Models}
The BP decoder has an equivalent Trellis representation that motivates the unfolding neural network architecture.
A simple example is provided in Figure~\ref{fig:bp}(b).
Each BP iteration $i$ unfolds into 2 hidden layers, $2\times i-1$ and $2\times i$, corresponding to two passes of messages from variable to check nodes and from check to variable nodes.
The number of nodes in each hidden layer is the same as the number of edges in the Tanner graph and, respectively, each node computes the message sent through each edge.
Thus, there are $2\times L$ hidden layers in this Trellis representation in addition to an input and output layer.
The input takes log-likelihood ratios of channel received signals and the output computes Eq.~\ref{eq:output}.

The unfolding neural network model shares the same architecture as the Trellis representation and adds trainable weights to the edges.
In other words, in odd layer $i$, the computation at node $i, e = (v,c)$, performs the following operation (activation function):
\begin{align}
	\label{eq:m_vc}
	x_{i, e = (v,c)} = w_{i,v}l_v + \sum_{e' = (c',v), c' \neq c} w_{i,e,e'}x_{i-1, e'}.
\end{align}
Note that trainable weights $w_{i,v}$ and $w_{i,e,e'}$ are introduced in the computation.
These weights can be trained and address various challenging obstacles with the BP method: 1) reduce the large number of iterations needed in BP, leading to more efficiency; 2) improve decoding performance and possibly approach optimal ML criterion, thanks to the ability to possibly minimize the effects of short cycles known to cause difficulties for BP decoders.

In even layer $i$, the computation at node $i, e = (v,c)$ is similar to that in the regular BP algorithm:
\begin{align}
	\label{eq:m_cv}
	x_{i, e = (c,v)} = 2 \tanh^{-1}\Big( \prod_{e' = (v',c), v' \neq v} \tanh \frac{x_{i-1,e'}}{2} \Big).
\end{align}
For numerical stability, we also apply normalization and truncation of messages after every layer.

Nodes at the output layer perform
\begin{align}
	\label{eq:o_v}
	o_v = \sigma \Big(w_{2L + 1,v}l_v + \sum_{e' = (c',v)} w_{2L+1,v,e'} x_{2L,e'} \Big),
\end{align}
where $\sigma(.)$ is the sigmoid function to obtain probability from the log-likelihood ratio representation.
Note that trainable weights $w_{2L + 1,v}$ and $w_{2L+1,v,e'}$ are also introduced here.


==> ECC_Globecom 2021_submit/preliminary4.tex <==
\section{Preliminaries}
\label{sec:prelim}
As the primary example of machine learning model in our paper, we describe in details the recent approach of unfolded belief propagation (BP) decoder. 
We first review the well known belief propagation (BP) decoder for error correcting codes and the deep neural network model that is constructed by unfolding this BP method.
Specifically, we summarize sum-product and min-sum algorithms along with their deep unfolding neural network models.

We consider the discrete-time additive white Gaussian noise (AWGN) channel model. In transmission time $i \in [1:n]$, the channel output is $Y_i = gX_i + Z_i$. where $g$ is the channel gain, $X_i \in \{ \pm 1\}$, $\{ Z_i \}$ is a WGN ($\sigma^2$) process, independent of the channel input $X^n = x^n(m)$, $m \in [1:2^{k}]$, and $k$ is the message length.

% \textbf{Channel noise model.} We consider a common channel model where additive random noise follows a Gaussian distribution with mean $0$ and variance $\sigma^2$, i.e., $N(0, \sigma^2)$.
% We follow the common assumption that transmitted codewords are uniformly selected at random from the set of all codewords.

\begin{figure}[!h]
	\centering
	%	\vspace{-0.1in}
	\includegraphics[width=\linewidth]{fig/bp_illustrate2.pdf}
	\caption{Tanner graph of a code and unfolded BP architecture based on code Trellis.}
	%	\vspace{-0.15in}
	\label{fig:bp}
\end{figure}
\subsection{Belief Propagation (BP) Decoder}

Given a linear error correcting code $C$ of block-length $n$, characterized by a parity check matrix $H$ of size $n \times (n-k)$, every codeword $x \in C$ satisfies $H^T x = 0$, where $H^T$ denotes the transpose of $H$ and $0$ the vector of $n-k$ zeros.
The BP decoder for a linear code can be constructed from the Tanner graph of the parity check matrix.
The Tanner graph contains $n-k$ check nodes and $n$ variable nodes arranged as a bipartite graph with edges between check and variable nodes, representing messages passing between these nodes.
If $H_{vc} = 1$, there is an edge between variable node $v$ and check node $c$.
% If $\mathbf{H}_{vc} = 1$, there is an edge between variable node $v$ and check node $c$.
A simple example is given in Figure~\ref{fig:bp}(a) with $n = 3$ variable nodes and $(n-k) = 2$ check nodes.
The BP decoder consists of multiple iterations.
Each iteration corresponds to one round of messaging passing between variable and check nodes.
In iteration $i$, on edge $e = (v,c)$, the message $x_{i, (v,c)}$ passed from variable node $v$ to the check node $c$ is given by
\begin{align}
	\label{eq:m_vc_bp}
	x_{i, e = (v,c)} = l_v + \sum_{e' = (c',v), c' \neq c} x_{i-1, e'},
\end{align}
where $l_v$ is the log-likelihood ratio of the channel output corresponding to the $v$th codeword bit $C_v$, i.e., $l_v = \log\frac{\Pr(C_v = 1 | y_v)}{\Pr(C_v = 0 | y_v)}$.
% Given random Gaussian noise,
%The log-likelihood ratio $l_v$ is
% \begin{align}
% 	l_v = \log\frac{\Pr(C_v = 1 | y_v)}{\Pr(C_v = 0 | y_v)}. \nonumber
% \end{align}

In the sum-product algorithm, the message $x_{i, (c,v)}$ from check node $c$ to variable node $v$ in iteration $i$ is computed as
\begin{align}
	\label{eq:m_cv_bp}
	x_{i, e = (c,v)} = 2 \tanh^{-1} \Bigg( \prod_{e' = (v',c), v' \neq v} \tanh \frac{x_{i,e'}}{2} \Bigg).
\end{align}
For numerical stability, the messages going into a node in both Eq.~(\ref{eq:m_vc_bp}) and Eq.~(\ref{eq:m_cv_bp}) are normalized at every iteration, and all the messages are also truncated within a fixed range.

Note that the computation in Eq.~(\ref{eq:m_cv_bp}) involves repeated multiplications and hyperbolic functions, which may lead to numerical problems in actual implementations. Even with truncation of message values within a certain range, e.g., commonly $[-10, 10]$, we still observe numerical problems when running the sum-product algorithm.
% Thus, we consider the Min-Sum algorithm in this paper.

% Note that the computation in Eq.~(\ref{eq:m_cv_bp}) involves repeated multiplications and hyperbolic functions, which may lead to heavy computation and numerical problems in actual implementations.
% Even with truncation of message values within a certain range, e.g., commonly $[-10, 10]$, we still observe numerical problems when running Sum-Product algorithm.

%\kwang{Truncate the messages from variable nodes to a check node into a specific range (e.g., -15.0 $\sim$ 15.0). It sets the size of the input messages in the check nodes to a level that does not cause numerical problems.}

The min-sum algorithm uses a ``min-sum'' approximation of the above message as follows:
\begin{align}
	x_{i, e = (c,v)} = \min_{e' = (v',c), v' \neq v} |x_{i,e'}| \prod_{e' = (v',c), v' \neq v} \sign(x_{i,e'}). \nonumber
\end{align}
Suppose the BP decoder runs $L$ iterations. Then the $v$th output after the final iteration is given by
\begin{align}
	\label{eq:output}
	o_v = l_v + \sum_{e' = (c',v)} x_{L,e'}.
\end{align}

\subsection{Unfolded BP Models}
The BP decoder has an equivalent Trellis representation that motivates the unfolding neural network architecture.
A simple example is provided in Figure~\ref{fig:bp}(b).
Each BP iteration $i$ unfolds into 2 hidden layers, $2i-1$ and $2i$, corresponding to two passes of messages from variable to check nodes and from check to variable nodes.
The number of nodes in each hidden layer is the same as the number of edges in the Tanner graph.
Each node computes a message sent through each edge.
Thus, there are $2\times L$ hidden layers in this Trellis representation in addition to input and output layers.
The input takes log-likelihood ratios of the received signal, and the output computes Eq.~\eqref{eq:output}.

The unfolding neural network model shares the same architecture as the Trellis representation and adds trainable weights to the edges.
In other words, in odd layer $i$, the computation at node $i, e = (v,c)$, performs the following operation (activation function):
\begin{align}
	\label{eq:m_vc}
	x_{i, e = (v,c)} = w_{i,v}l_v + \sum_{e' = (c',v), c' \neq c} w_{i,e,e'}x_{i-1, e'}.
\end{align}
Note that trainable weights $w_{i,v}$ and $w_{i,e,e'}$ are introduced in the computation.
These weights can be trained and address various challenging obstacles with the BP method: 1) reduce the large number of iterations needed in BP, leading to higher efficiency; 2) improve decoding performance and possibly approach optimal criterion, thanks to the ability to minimize the effects of short cycles in the Tanner graph known to cause difficulties for BP decoders.

In even layer $i$, the computation at node $i, e = (c,v)$ is similar to that in the regular BP algorithm:
\begin{align}
	\label{eq:m_cv}
	x_{i, e = (c,v)} = 2 \tanh^{-1} \Bigg( \prod_{e' = (v',c), v' \neq v} \tanh \frac{x_{i-1,e'}}{2} \Bigg).
\end{align}
For numerical stability, we usually apply truncation of messages after every layer.

Nodes at the output layer perform
\begin{align}
	\label{eq:o_v}
	o_v = \sigma \Bigg(w_{2L + 1,v}l_v + \sum_{e' = (c',v)} w_{2L+1,v,e'} x_{2L,e'} \Bigg),
\end{align}
where $\sigma(\cdot)$ is the sigmoid function to obtain probability from the log-likelihood ratio representation.
Note that trainable weights $w_{2L + 1,v}$ and $w_{2L+1,v,e'}$ are also introduced here.


==> algorithm1.tex <==
\section{Proposed model}
\label{sec:alg}

Motivated by the generative adversarial network (GAN), our proposed model combines deep unfolding neural network model with a discriminator that distinguishes between valid codewords and outputs of the unfolding model. The decoder and discriminator competes in game: the decoder tries to fool the discriminator in thinking that its outputs are valid codes, or, maximize the classification error; on the other hand, the discriminator is a classification model that tries to tell which inputs are original valid codes and which are generated by the decoder. Effectively, the two models improve each other at the same time as the better decoder or discriminator gives better feedback to the other of how to improve.

==> algorithm2.tex <==
\section{Proposed model}
\label{sec:alg}

Motivated by the recent advances in GANs, we propose to combine deep unfolding neural network models with a discriminator that distinguishes between codewords following the uniform distribution and decoded outputs of the unfolding network.
The decoder and discriminator compete in a zero-sum game: the decoder tries to fool the discriminator into thinking that its outputs are codewords, i.e., maximizing the classification error; on the other hand, the discriminator is a classification model that tries to tell which input sequences are original codewords and which are generated by the decoder.
Effectively, the two models improve at the same time as the better decoder or discriminator gives better feedback to the other about how to improve to better compete.

\subsection{Model architecture}
\begin{figure}[!h]
	\centering
	\vspace{-0.1in}
	\includegraphics[width=1\linewidth]{fig/proposed_model_l.pdf}
	\vspace{-0.1in}
	\caption{Proposed model architecture where decoder and discriminator networks compete and improve together as both are trained till equilibrium.}
	\label{fig:proposed_model}
\end{figure}

The proposed model is described in Figure~\ref{fig:proposed_model}.
The BP unfolded decoder network $G$ takes the received noisy signal from the channel and produces the decoded output $\hat \x$. The discriminator network $D$ is a classification model and aims at discriminating between codewords $\x$ and decoded outputs $\hat \x$ from the decoder.
The cost function $f(G,D)$ evaluates how well the discriminator network performs.
Thus, the goal of decoder is the opposite with that of the discriminator, which is maximizing the loss function.

Let $\mathcal{U}$ denote the uniform distribution generating random codewords and $\mathcal{P}_G$ the resulting distribution of the decoder's outputs. We overload the notations $\mathcal{U}$ and $\mathcal{P}_G$ to denote both the distribution and probability mass function.
We use the following common loss function in generative adversarial networks:
\begin{align}
	\label{eq:f_gd}
	f(G,D) = \mathbb{E}_{\x \sim \mathcal{U}} [\log D(\x)] + \mathbb{E}_{\y \sim \mathcal{P}_G} [\log(1 - D(\y))].
\end{align}
This function measures how well the discriminator classifies codewords from decoded outputs.
In other words, the discriminator tries to maximize this function while the decoder aims at minimizing it.
Hence, the optimization problem is to find $G^*$ and $D^*$ that solve the following min-max problem:
\begin{align}
	\label{eq:opt_problem}
	\min_{G}\max_{D} \mathbb{E}_{\x \sim \mathcal{U}} [\log D(\x)] + \mathbb{E}_{\y \sim \mathcal{P}_G} [\log (1 - D(\y))],
\end{align}
where $G$ is the BP unfolded network with parameters $w_{i,v}, w_{i,e,e'}$ and $w_{2L+1,v,e'}$, and $D$ is a classification model within some class of models.
As we will show later, with different classes of classification models, we can prove various results regarding the equilibrium between decoder and discriminator with respect to the min-max game in Eq.~(\ref{eq:opt_problem}).

\subsection{Theoretical results}

\subsubsection{Approaching optimal maximum likelihood performance}
\label{subsec:approach_ml}

We first prove that our model has a strong connection with the optimal ML decoder that is computationally intractable in practice due to its hardness.
We show that the ML decoder along with a discriminator trained with the ML decoder is in fact an equilibrium of our min-max game defined in Eq.~(\ref{eq:opt_problem}).
Let $G_{ML}$ represent the optimal ML decoder and $D_{ML}$ be defined as follows:
\begin{align}
	\label{eq:dml_prob}
	D_{ML} = \argmax_{D} \mathbb{E}_{\x \sim \mathcal{U}} [\log D(\x)] + \mathbb{E}_{\y \sim \pgml} [\log (1 - D(\y))].
\end{align}
Note that $D$ is in the class of all possible classification models.

From \cite{goodfellow2014generative}, we have the following lemma characterizing $\dml$ based on $\gml$.
\begin{lemma}
	\label{lem:dml_opt}
	Let $D$ be from the class of all classification models.
	The solution $\dml$ for problem (\ref{eq:dml_prob}) with respect to fixing $G$ to be $\gml$, i.e., having distribution $\pgml$, is
	\begin{align}
		\dml(x) = \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}, \forall \x \in \mathbb{C}.
	\end{align}
\end{lemma}

We establish the following theorem showing that $\gml$ and $\dml$ form an equilibrium of our min-max problem in (\ref{eq:opt_problem}).
\begin{theorem}
	\label{theo:ml_equi}
	The optimal ML decoder $\gml$ and the corresponding discriminator $\dml$ form an equilibrium for our min-max problem in (\ref{eq:opt_problem}).
	Specifically, we have
	\begin{align}
%		\label{eq:ml_equi}
		\max_{D} f(\gml, D) \leq f(\gml, \dml) \leq \min_{G} f(G, \dml), \nonumber
	\end{align}
	where $f(G,D)$ is defined in Eq.~(\ref{eq:f_gd}) and $G$ is from the class of all unfolded BP networks with different weight parameters $w_{i,v}, w_{i,e,e'}$ and $w_{2L+1,v,e'}$ as defined in Eq.~(\ref{eq:m_vc}) and Eq.~(\ref{eq:o_v}).
\end{theorem}
\begin{proof}$ $
	
	The first inequality $\max_{D} f(\gml, D) \leq f(\gml, \dml)$ follows immediately from the definition of $\dml$ in Lemma~\ref{lem:dml_opt} that $\dml$ is the optimal classification model with respect to the optimal ML decoder $\gml$.
	
	To prove the second inequality $f(\gml, \dml) \leq \min_{G} f(G, \dml)$, consider the function $f(G, \dml)$.
	We have
	\begin{align}
		\label{eq:14}
		f(G, \dml) &= \mathbb{E}_{\x \sim \mathcal{U}} [\log \dml(\x)] + \mathbb{E}_{\y \sim \mathcal{P}_G} [\log (1 - \dml(\y))] \nonumber \\
		& = \mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\ 
		& \qquad + \mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log (1 - \frac{\mathcal{U}(\y)}{\mathcal{U}(\y) + \pgml(\y)})\right] \nonumber \\
		& = \mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
		& \qquad + \mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right].
	\end{align}

	Regarding the optimization problem of $f(G, \dml)$ over $G$, the first term in Eq.~(\ref{eq:14}) is fixed for all $G$ and we can focus on the second term with $\y \sim \mathcal{P}_G$.
	For any $\y \not\in \mathbb{C}$ and $\pgml(\y) \neq 0$, $\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}$ achieves its maximum value of $0$ since $\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)} \leq 0$.
	Therefore, to minimize $f(G,\dml)$, we can narrow our consideration to decoders that produce only codewords.
	Furthermore, due to the symmetry of linear block codes, $\pgml$ is the uniform distribution over codewords.
	Thus, for any decoder $G$ that only produces codewords, we have
	\begin{align}
		\label{eq:15}
		& \mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right] \nonumber \\ 
		& = \mathbb{E}_{\y \sim \pgml} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right] = \log \frac{1}{2}.
	\end{align}
	
	Taking the minimization over all BP unfolding networks $G$ in Eq.~(\ref{eq:14}) and incorporating Eq.~(\ref{eq:15}) into Eq.~(\ref{eq:14}), we obtain
	\begin{align}
		\min_{G} f(G, \dml) & = \min_{G} \Big(\mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
		& \text{ \ \ } + \mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right] \Big) \nonumber \\
		& \geq \mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
		& \text{ \ \ } + \min_{G} \left(\mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right]\right) \nonumber \\
		& = \mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
		& \text{ \ \ } + \mathbb{E}_{\y \sim \pgml} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right] \nonumber \\
		& = f(\gml, \dml).
	\end{align}
	That completes the proof of the second inequality and the theorem.
%	We rewrite the term of interest as follows:
%	\begin{align}
%		\mathbb{E}_{y \sim \mathcal{P}_G} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right] = \mathbb{E}_{x \sim \mathcal{U}, r \sim \mathcal{G}(0, \sigma^2)} \left[ \log \frac{\pgml(G(x+r))}{\mathcal{U}(G(x+r)) + \pgml(G(x+r))} \right],
%	\end{align}
%	where $r \sim \mathcal{G}(0, \sigma^2)$ is the random noise following the Gaussian distribution with mean $0$ and variance $\sigma^2$.
\end{proof}

The equilibrium point corresponding to the optimal ML decoder suggests that if we train our BP unfolding network till convergence to an equilibrium, we can possibly achieve the optimal ML decoding performance.
This possibility is high for the BP unfolding network since the original BP method is based on the Tanner graph of the code and the resulting BP solution also provides good approximations of the true likelihood over codewords in practice.

\subsubsection{Model simplification and preserving BP fixed points}
\label{subsec:bp_fixed}

The number of weight parameters in the deep unfolding model is quite large, i.e., $O(L\cdot n + L\cdot E \cdot d_{max})$, where $L$ is the number of BP iterations, $E$ is the number of edges in the Tanner graph, and $d_{\max}$ denotes the maximum degree of any node.
We can improve the efficiency of our model by weight simplification.
%the following weight simplification scheme, motivated from practical observations, which also brings in another theoretical property. 
We simplify the weight parameters $w_{i,v}$ and $w_{i,e,e'}$ of layer $i$ in the unfolding network into a single weight parameter $w_i$ and reduce the total number of trainable weights to $L$.
This stems from our experimental observations that most of the parameters in the same layer have similar values after training.
Intuitively, this simplification helps reduce the computation in both training and running the model. 

The BP method on factor graphs has been studied extensively in the literature \cite{yedidia2001characterization,yedidia2003understanding,kuck2020belief,satorras2020neural} and shown to have interesting properties.
Among those properties, an important one is the correspondence of BP fixed points to solutions of the Bethe free energy defined on the factor graph \cite{yedidia2001characterization,yedidia2003understanding}.
The solutions minimizing the Bethe free energy provide a lower-bound for the factor graph's partition function, which is useful for inferences on the graph.
A set of messages is a fixed point of BP if they remain the same values after updates in Eq.~(\ref{eq:m_vc_bp}) and Eq.~(\ref{eq:m_cv_bp}).
We can derive a variant of our model that preserves all the fixed points of BP method in a straightforward manner.
Specifically, let $\bar{x}_{i,e=(v,c)}$ be the updated message from variable node $v$ to check node $c$ for the original BP method in Eq.~(\ref{eq:m_vc_bp}).
The activation function in odd layer $i$ is modified to
\begin{align}
	\label{eq:m_vc_variant}
	x_{i, e = (v,c)} = & (\bar{x}_{i,e} - \bar{x}_{i-1,e}) \Big[w_{i,v}l_v \nonumber \\
	& + \sum_{e' = (c',v), c' \neq c} w_{i,e,e'}x_{i-1, e'}\Big] + \bar{x}_{i-1,e}.
\end{align}
The activation function on the even layers are the same as in the original model, i.e., Eq.~(\ref{eq:m_cv}).

%More importantly, it leads to a critical theoretical result that the BP unfolding network preserves all the fixed point solutions of the original BP method. Thus, our simplified model inherits all the interesting theoretical properties of BP method including its correspondence of fixed points to solutions of Bethe approximation \cite{yedidia2001characterization,yedidia2003understanding}, which provides a lower-bound for the factor graph's partition function in our case.

We obtain the following result regarding the relation between BP fixed points and our simplified deep unfolding model.

\begin{proposition}
	The simple variant of the deep unfolding network with activation function in Eq.~(\ref{eq:m_vc_variant}) preserves all the fixed points of the original belief propagation (BP) method.
\end{proposition}
\begin{proof}
	The proof is evident from the definition of fixed points.
	The set of $\bar{x}_{i,e=(v,c)}$ and $\bar{x}_{i,(e = (c,v))}$ is a fixed point of BP if $\bar{x}_{i,e=(v,c)} = \bar{x}_{i-1,e=(v,c)}$ and $\bar{x}_{i,(e = (c,v))} = \bar{x}_{i-1,(e = (c,v))}$ for all $(c,v)$ and $(v,c)$.
	Plugging these conditions into the activation functions of our model variant in Eq.~(\ref{eq:m_cv}) and Eq.~(\ref{eq:m_vc_variant}), we also obtain the same conditions for fixed points that $x_{i,e=(v,c)} = x_{i-1,e=(v,c)} = \bar{x}_{i-1,e=(v,c)}$ and $x_{i,(e = (c,v))} = x_{i-1,(e = (c,v))} = \bar{x}_{i-1,(e = (c,v))}$.
	Hence, any fixed point of BP is also a fixed point of our model.
\end{proof}

\subsection{Online training for channel dynamics adaptation}

Compared to the deep unfolding model by itself, an advantageous characteristic of our game model is that it only requires received noisy signals from the channel and codewords which can be generated uniformly using the generator matrix of the code.
This property makes our model amenable to online training and effectively adapting to channel dynamics.
Specifically, we can collect batches of received signals and generate random batches of codewords to continually train our model on the fly.
This is in contrast to the deep unfolding model alone, which requires both the channel noisy signals and the true transmitted codewords to train it.

%\kwang{We will add details about GAN specifically designed for our model.}

%Summary of technical results (12/14/2020):
%\begin{itemize}
%    \item For weight simplification scheme that uses 1 single trainable weight value in each layer, we can show that this simplified model preserves fixed point solutions of the original belief propagation (BP) algorithm. Since the original BP's fixed point solution solves Bethe approximation, our model also has this property and can potentially do better theoretically thanks to trainable weight values. Also, because of solving Bethe approximation, showing the correspondence to ML optimal criteria is hard.
%    \item Our combination with GAN actually drives the deep unfolding network towards ML optimal criteria by enforcing a necessary condition of being ML optimal, that is the average of model output distribution must be uniform. Imagine each noisy input gives a distribution over valid codewords and if we average out all the distributions for all possible noisy inputs, ML optimal criteria gives us a uniform distribution. This property is provided by GAN property at equilibrium.
%\end{itemize}

==> algorithm3.tex <==
\section{Proposed Model}
\label{sec:alg}

Motivated by the recent advances in GANs, we propose to combine deep unfolding neural network models with a discriminator that distinguishes between codewords following the uniform distribution and decoded outputs of the unfolding network.
The decoder and discriminator compete in a zero-sum game: the decoder tries to fool the discriminator into thinking that its outputs are codewords, i.e., maximizing the classification error; on the other hand, the discriminator is a classification model that tries to tell which input sequences are original codewords and which are generated by the decoder.
Effectively, the two models improve at the same time as the better decoder or discriminator gives better feedback to the other about how to improve to better compete.

\subsection{Model Architecture}
\begin{figure}[!t]
	\centering
	\vspace{-0.15in}
	\includegraphics[width=0.9\linewidth]{fig/proposed_model_l.pdf}
%	\vspace{-0.1in}
	\caption{Proposed model architecture where decoder and discriminator networks compete and improve together as both are trained till equilibrium.}
	\vspace{-0.15in}
	\label{fig:proposed_model}
\end{figure}

The proposed model is described in Figure~\ref{fig:proposed_model}.
The BP unfolded decoder network $G$ takes the received noisy signal from the channel and produces the decoded output $\hat \x$. The discriminator network $D$ is a classification model and aims at discriminating between codewords $\x$ and decoded outputs $\hat \x$ from the decoder.
The cost function $f(G,D)$ evaluates how well the discriminator network performs.
Thus, the goal of decoder is the opposite with that of the discriminator, which is maximizing the loss function.

Let $\mathcal{U}$ denote the uniform distribution generating random codewords and $\mathcal{P}_G$ the resulting distribution of the decoder's outputs.
Here, we slightly abuse notation and use $\mathcal{U}$ and $\mathcal{P}_G$ to denote both a distribution and a probability mass function.
We use the following common loss function in generative adversarial networks:
\begin{align}
	\label{eq:f_gd}
  f(G,D) = \mathbb{E}_{x \sim \mathcal{U}} [\log D(x)] + \mathbb{E}_{y \sim \mathcal{P}_G} [\log(1 - D(y))].
	% f(G,D) = \mathbb{E}_{\x \sim \mathcal{U}} [\log D(\x)] + \mathbb{E}_{\y \sim \mathcal{P}_G} [\log(1 - D(\y))].
\end{align}
This function measures how well the discriminator classifies codewords from decoded outputs.
In other words, the discriminator tries to maximize this function while the decoder aims at minimizing it.
Hence, the optimization problem is to find $G^*$ and $D^*$ that solve the following min-max problem:
\begin{align}
	\label{eq:opt_problem}
  \min_{G}\max_{D} \mathbb{E}_{x \sim \mathcal{U}} [\log D(x)] + \mathbb{E}_{y \sim \mathcal{P}_G} [\log (1 - D(y))],
	% \min_{G}\max_{D} \mathbb{E}_{\x \sim \mathcal{U}} [\log D(\x)] + \mathbb{E}_{\y \sim \mathcal{P}_G} [\log (1 - D(\y))],
\end{align}
where $G$ is the BP unfolded network with parameters $w_{i,v}, w_{i,e,e'}$ and $w_{2L+1,v,e'}$, and $D$ is a classification model within some class of models.
As we will show later, with different classes of classification models, we can prove various results regarding the equilibrium between decoder and discriminator with respect to the min-max game in Eq.~(\ref{eq:opt_problem}).

\subsection{Theoretical Results}

\subsubsection{Approaching optimal maximum likelihood performance}
\label{subsec:approach_ml}
We first prove that our model has a strong connection with the optimal ML decoder that is computationally intractable in practice due to its hardness.
We show that the ML decoder along with a discriminator trained with the ML decoder is in fact an equilibrium of our min-max game defined in Eq.~(\ref{eq:opt_problem}).
Let $G_{ML}$ represent the optimal ML decoder and $D_{ML}$ be defined as follows:
\begin{align}
	\label{eq:dml_prob}
  D_{ML} = \argmax_{D} \mathbb{E}_{x \sim \mathcal{U}} [\log D(x)] + \mathbb{E}_{y \sim \pgml} [\log (1 - D(y))].
	% D_{ML} = \argmax_{D} \mathbb{E}_{\x \sim \mathcal{U}} [\log D(\x)] + \mathbb{E}_{\y \sim \pgml} [\log (1 - D(\y))].
\end{align}
Note that $D$ is in the class of all possible classification models.

From \cite{goodfellow2014generative}, we have the following lemma characterizing $\dml$ based on $\gml$.
\begin{lemma}
	\label{lem:dml_opt}
	Let $D$ be from the class of all classification models.
	The solution $\dml$ for problem (\ref{eq:dml_prob}) with respect to fixing $G$ to be $\gml$, i.e., having distribution $\pgml$, is
	\begin{align}
    \dml(x) = \frac{\mathcal{U}(x)}{\mathcal{U}(x) + \pgml(x)}, ~ x \in C. \nonumber
		% \dml(x) = \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}, \forall \x \in \mathbb{C}. \nonumber
	\end{align}
\end{lemma}

We establish the following theorem showing that $\gml$ and $\dml$ form an equilibrium of our min-max problem in (\ref{eq:opt_problem}).
\begin{theorem}
	\label{theo:ml_equi}
	The optimal ML decoder $\gml$ and the corresponding discriminator $\dml$ form an equilibrium for our min-max problem in (\ref{eq:opt_problem}).
	Specifically, we have
	\begin{align}
%		\label{eq:ml_equi}
		\max_{D} f(\gml, D) \leq f(\gml, \dml) \leq \min_{G} f(G, \dml), \nonumber
	\end{align}
	where $f(G,D)$ is defined in Eq.~(\ref{eq:f_gd}) and $G$ is from the class of all unfolded BP networks with different weight parameters $w_{i,v}, w_{i,e,e'}$ and $w_{2L+1,v,e'}$ as defined in Eq.~(\ref{eq:m_vc}) and Eq.~(\ref{eq:o_v}).
\end{theorem}
\begin{proof}
	The first inequality $\max_{D} f(\gml, D) \leq f(\gml, \dml)$ follows immediately from the definition of $\dml$ in Lemma~\ref{lem:dml_opt} that $\dml$ is the optimal classification model with respect to the optimal ML decoder $\gml$.

	To prove the second inequality $f(\gml, \dml) \leq \min_{G} f(G, \dml)$, consider the function $f(G, \dml)$.
	We have
  \begin{align}
		\label{eq:14}
		f(G, \dml) &= \mathbb{E}_{x \sim \mathcal{U}} [\log \dml(x)] + \mathbb{E}_{y \sim \mathcal{P}_G} [\log (1 - \dml(y))] \nonumber \\
		& = \mathbb{E}_{x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(x)}{\mathcal{U}(x) + \pgml(x)}\right] \nonumber \\
		& \qquad + \mathbb{E}_{y \sim \mathcal{P}_G} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right].
	\end{align}
	% \begin{align}
	% 	\label{eq:14}
	% 	f(G, \dml) &= \mathbb{E}_{\x \sim \mathcal{U}} [\log \dml(\x)] + \mathbb{E}_{\y \sim \mathcal{P}_G} [\log (1 - \dml(\y))] \nonumber \\
	% 	% & = \mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
	% 	% & \qquad + \mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log (1 - \frac{\mathcal{U}(\y)}{\mathcal{U}(\y) + \pgml(\y)})\right] \nonumber \\
	% 	& = \mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
	% 	& \qquad + \mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right].
	% \end{align}

	Regarding the optimization problem of $f(G, \dml)$ over $G$, the first term in Eq.~(\ref{eq:14}) is fixed for all $G$ and we can focus on the second term with $y \sim \mathcal{P}_G$.
	For any $y \not\in C$ and $\pgml(y) \neq 0$, $\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}$ achieves its maximum value of $0$ since $\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)} \leq 0$.
	Therefore, to minimize $f(G,\dml)$, we can narrow our consideration to decoders that produce only codewords.
	Furthermore, due to the symmetry of linear block codes, $\pgml$ is the uniform distribution over codewords.
	Thus, for any decoder $G$ that only produces codewords, we have
	\begin{align}
		\label{eq:15}
    & \mathbb{E}_{y \sim \mathcal{P}_G} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right] \nonumber \\
		& = \mathbb{E}_{y \sim \pgml} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right] = \log \frac{1}{2}.
		% & \mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right] \nonumber \\
		% & = \mathbb{E}_{\y \sim \pgml} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right] = \log \frac{1}{2}.
	\end{align}

	Taking the minimization over all BP unfolding networks $G$ in Eq.~(\ref{eq:14}) and incorporating Eq.~(\ref{eq:15}) into Eq.~(\ref{eq:14}), we obtain
	\begin{align}
    \min_{G} f(G, \dml) & = \min_{G} \Big(\mathbb{E}_{x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(x)}{\mathcal{U}(x) + \pgml(x)}\right] \nonumber \\
		& \text{ \ \ } + \mathbb{E}_{y \sim \mathcal{P}_G} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right] \Big) \nonumber \\
		& = \mathbb{E}_{x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(x)}{\mathcal{U}(x) + \pgml(x)}\right] \nonumber \\
		& \text{ \ \ } + \min_{G} \left(\mathbb{E}_{y \sim \mathcal{P}_G} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right]\right) \nonumber \\
		& = \mathbb{E}_{x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(x)}{\mathcal{U}(x) + \pgml(x)}\right] \nonumber \\
		& \text{ \ \ } + \mathbb{E}_{y \sim \pgml} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right] \nonumber \\
		& = f(\gml, \dml).
		% \min_{G} f(G, \dml) & = \min_{G} \Big(\mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
		% & \text{ \ \ } + \mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right] \Big) \nonumber \\
		% & \geq \mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
		% & \text{ \ \ } + \min_{G} \left(\mathbb{E}_{\y \sim \mathcal{P}_G} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right]\right) \nonumber \\
		% & = \mathbb{E}_{\x \sim \mathcal{U}} \left[\log \frac{\mathcal{U}(\x)}{\mathcal{U}(\x) + \pgml(\x)}\right] \nonumber \\
		% & \text{ \ \ } + \mathbb{E}_{\y \sim \pgml} \left[\log \frac{\pgml(\y)}{\mathcal{U}(\y) + \pgml(\y)}\right] \nonumber \\
		% & = f(\gml, \dml).
	\end{align}
	That completes the proof of the second inequality and the theorem.
%	We rewrite the term of interest as follows:
%	\begin{align}
%		\mathbb{E}_{y \sim \mathcal{P}_G} \left[\log \frac{\pgml(y)}{\mathcal{U}(y) + \pgml(y)}\right] = \mathbb{E}_{x \sim \mathcal{U}, r \sim \mathcal{G}(0, \sigma^2)} \left[ \log \frac{\pgml(G(x+r))}{\mathcal{U}(G(x+r)) + \pgml(G(x+r))} \right],
%	\end{align}
%	where $r \sim \mathcal{G}(0, \sigma^2)$ is the random noise following the Gaussian distribution with mean $0$ and variance $\sigma^2$.
\vspace{-0.05in}
\end{proof}

The equilibrium point corresponding to the optimal ML decoder suggests that if we train our BP unfolding network till convergence to an equilibrium, we can possibly achieve the optimal ML decoding performance.
This possibility is high for the BP unfolding network since the original BP method is based on the Tanner graph of the code and the resulting BP solution also provides good approximations of the true likelihood over codewords in practice.

\subsubsection{Preserving BP fixed points}
The BP method on factor graphs has been studied extensively in the literature \cite{yedidia2001characterization,yedidia2003understanding,kuck2020belief,satorras2020neural} and shown to have interesting properties.
Among those properties, an important one is the correspondence of BP fixed points to solutions of the Bethe free energy defined on the factor graph \cite{yedidia2001characterization,yedidia2003understanding}.
The solutions minimizing the Bethe free energy provide a lower-bound for the factor graph's partition function, which is useful for inferences on the graph.
A set of messages is a fixed point of BP if they remain the same values after updates in Eq.~(\ref{eq:m_vc_bp}) and Eq.~(\ref{eq:m_cv_bp}).
We can derive a variant of our model that preserves all the fixed points of BP method in a straightforward manner.
Specifically, let $\bar{x}_{i,e=(v,c)}$ be the updated message from variable node $v$ to check node $c$ for the original BP method in Eq.~(\ref{eq:m_vc_bp}).
The activation function in odd layer $i$ is modified to
\vspace{-0.05in}
\begin{align}
	\label{eq:m_vc_variant}
	x_{i, e = (v,c)} = & (\bar{x}_{i,e} - \bar{x}_{i-1,e}) \Big[w_{i,v}l_v \nonumber \\
	& + \sum_{e' = (c',v), c' \neq c} w_{i,e,e'}x_{i-1, e'}\Big] + \bar{x}_{i-1,e}.
\end{align}
The activation function on the even layers are the same as in the original model, i.e., Eq.~(\ref{eq:m_cv}).

%More importantly, it leads to a critical theoretical result that the BP unfolding network preserves all the fixed point solutions of the original BP method. Thus, our simplified model inherits all the interesting theoretical properties of BP method including its correspondence of fixed points to solutions of Bethe approximation \cite{yedidia2001characterization,yedidia2003understanding}, which provides a lower-bound for the factor graph's partition function in our case.

We obtain the following result regarding the relation between BP fixed points and our simplified deep unfolding model.

\begin{proposition}
	The simple variant of the deep unfolding network with activation function in Eq.~(\ref{eq:m_vc_variant}) preserves all the fixed points of the original belief propagation (BP) method.
\end{proposition}
\begin{proof}
	The proof is evident from the definition of fixed points.
	The set of $\bar{x}_{i,e=(v,c)}$ and $\bar{x}_{i,(e = (c,v))}$ is a fixed point of BP if $\bar{x}_{i,e=(v,c)} = \bar{x}_{i-1,e=(v,c)}$ and $\bar{x}_{i,(e = (c,v))} = \bar{x}_{i-1,(e = (c,v))}$ for all $(c,v)$ and $(v,c)$.
	Plugging these conditions into the activation functions of our model variant in Eq.~(\ref{eq:m_cv}) and Eq.~(\ref{eq:m_vc_variant}), we also obtain the same conditions for fixed points that $x_{i,e=(v,c)} = x_{i-1,e=(v,c)} = \bar{x}_{i-1,e=(v,c)}$ and $x_{i,(e = (c,v))} = x_{i-1,(e = (c,v))} = \bar{x}_{i-1,(e = (c,v))}$.
	Hence, any fixed point of BP is also a fixed point of our model.
\end{proof}
\subsubsection{Model simplification}
% \subsubsection{Model simplification and preserving BP fixed points}
\label{subsec:bp_fixed}

The number of weight parameters in the deep unfolding model is quite large, i.e., $O(L\cdot n + L\cdot E \cdot d_{max})$, where $L$ is the number of BP iterations, $E$ is the number of edges in the Tanner graph, and $d_{\max}$ denotes the maximum degree of any node.
We can improve the efficiency of our model by weight simplification.
%the following weight simplification scheme, motivated from practical observations, which also brings in another theoretical property.
We simplify the weight parameters $w_{i,v}$ and $w_{i,e,e'}$ of layer $i$ in the unfolding network into a single weight parameter $w_i$ and reduce the total number of trainable weights to $L$.
This stems from our experimental observations that most of the parameters in the same layer have similar values after training.
Intuitively, this simplification helps reduce the computation in both training and running.

\subsection{Online training for channel dynamics adaptation}

Compared to the deep unfolding model by itself, an advantageous characteristic of our game model is that it only requires received noisy signals from the channel and codewords which can be generated uniformly using the generator matrix of the code.
This property makes our model amenable to online training and effectively adapting to channel dynamics.
Specifically, we can collect batches of received signals and generate random batches of codewords to continually train our model on the fly.
This is in contrast to the deep unfolding model alone, which requires both the channel noisy signals and the true transmitted codewords to train it.

%\kwang{We will add details about GAN specifically designed for our model.}

%Summary of technical results (12/14/2020):
%\begin{itemize}
%    \item For weight simplification scheme that uses 1 single trainable weight value in each layer, we can show that this simplified model preserves fixed point solutions of the original belief propagation (BP) algorithm. Since the original BP's fixed point solution solves Bethe approximation, our model also has this property and can potentially do better theoretically thanks to trainable weight values. Also, because of solving Bethe approximation, showing the correspondence to ML optimal criteria is hard.
%    \item Our combination with GAN actually drives the deep unfolding network towards ML optimal criteria by enforcing a necessary condition of being ML optimal, that is the average of model output distribution must be uniform. Imagine each noisy input gives a distribution over valid codewords and if we average out all the distributions for all possible noisy inputs, ML optimal criteria gives us a uniform distribution. This property is provided by GAN property at equilibrium.
%\end{itemize}


==> conc.tex <==
\section{Conclusion}

We have proposed a game-theoretic framework that combines a decoder network with a discriminator, which compete in a zero-sum game.
The decoder tries to decode a received noisy signal from the communication channel while the discriminator tries to distinguish between codewords from the decoded words.
Both decoder and discriminator improve together to be better at their own tasks.
We show a strong connection between our model and the optimal maximum likelihood (ML) decoder as the ML decoder forms a Nash equilibrium in our game model.
Our experimental results confirm improved decoding performance compared to the recent deep learning models and the belief propagation method.

%\section*{Acknowledgements}
%This research was, in part, funded by the U.S. Government, Defense Advanced Research Projects Agency (DARPA) under contract no. HR00112090056.
%The views and conclusions contained in this document are those of the authors and should not be interpreted as representing the official policies, either expressed or implied, of the U.S. Government.

==> experiments1.tex <==
\section{Experiments}
We apply our model on decoding of BCH and Reed Solomon codes and compare the results to that of deep unfolding model.

\subsection{Setting}
We use the same deep unfolding model as in \cite{nachmani2018deep} that corresponds to 5 BP iterations and add a simple 2 layer fully connected layers discriminator with the hidden layer having size of 1024 and sigmoid activation function and output layer being a single neuron. We applied Adam optimizer with learning rate of 0.001 and batch size 64. 10000 codes are used for training and 100000 codes are for testing. We consider AWGN channel with various signal-to-noise (SNR) ratios.

\subsection{Results}
\begin{figure}[!h]
	\centering
	\includegraphics[width=0.7\linewidth]{fig/FER_15_11_log.png}
	\caption{FER results on BCH(15,11).}
	\label{fig:bch_15_11}
\end{figure}

==> experiments2.tex <==
\section{Experiments}
\label{sec:exps}

We demonstrate the better decoding performance of our model in comparison with the original deep unfolding network and BP decoder on various codes.

\begin{figure}[!t]
	\centering
	\begin{subfigure}[b]{0.8\linewidth}
		\includegraphics[width=\linewidth]{fig/bch_15_11}
		\caption{BCH(15,11)}
	\end{subfigure}
	\begin{subfigure}[b]{0.8\linewidth}
		\includegraphics[width=\linewidth]{fig/bch_63_45}
		\caption{BCH(63,45)}
	\end{subfigure}
	%\includegraphics[width=0.7\linewidth]{fig/bch_15_11}
	\caption{Performance of different decoders on BCH code.}
	\label{fig:bch_fer}
\end{figure}
\begin{figure}[!t]
	\centering
	\begin{subfigure}[b]{0.8\linewidth}
		\includegraphics[width=\linewidth]{fig/rs_15_11}
		\caption{RS(15,11)}
	\end{subfigure}
	\begin{subfigure}[b]{0.8\linewidth}
		\includegraphics[width=\linewidth]{fig/rs_31_27}
		\caption{RS(31,27)}
	\end{subfigure}
	%\includegraphics[width=0.7\linewidth]{fig/bch_15_11}
	\caption{Performance of different decoders of Reed-Solomon codes (SSID is an effective belief propagation method for RS).}
	\label{fig:rs_fer}
\end{figure}

\subsection{Setting}
We tested on both BCH codes BCH(15,11), BCH(63,45), and Reed-Solomon codes RS(15,11), RS(31,27), with an AWGN channel and various signal-to-noise (SNR) ratios.
For BCH codes, we use the neural offset min-sum deep unfolding model, FNOMS, as in \cite{nachmani2018deep} that unfolds 5 BP iterations and adds a discriminator with two fully connected layers, each of size 1024 with sigmoid activation function, and a single neuron output layer.
For Reed-Solomon codes, the decoder network, namely DeepSSID, unfolds the Stochastic Shifting Based Iterative Decoding (SSID) model\cite{zhang2020iterative}.
We applied the Adam optimizer with learning rate of 0.001 for both decoder and discriminator training and batch size 64.
10000 and 100000 codewords are randomly drawn for training and testing, respectively.

%\kwang{Compare with the classic results of BCH codes with BP decoding. Provide the number of iterations for decoding for all schemes.}
%\kwang{As commented in the previous section, use truncation for the sum-product algorithm rather than the min-sum algorithm for a fair comparison with \cite{nachmani2018deep}. In general, the sum-product algorithm outperforms the min-sum algorithm.}

\subsection{Results}

We compare our model, denoted by \method, with the original deep unfolding model and BP method with 100 iterations.
The results are demonstrated in Figure~\ref{fig:bch_fer} for BCH codes and Figure~\ref{fig:rs_fer} for Reed-Solomon codes.
In both cases, the results show that \method{} achieves improved decoding performance compared to both previous deep unfolding networks and BP.
The improvement is approximately 0.5dB consistently across all signal-to-noise ratios and different codes.

Notably, the improvement of \method{} for shorter block length as in BCH(15,11) and RS(15,11) is more significant than for longer block length as in BCH(63,45) and RS(31,27).
This is possibly due to the fixed number of layers in the decoder network and suggests larger block codes may need more layers or deeper networks to perform well.

%Weight patterns when training in GAN model:
%\begin{figure}[!h]
%	\centering
%	\includegraphics[width=0.5\linewidth]{fig/gan_weight_pattern.png}
%	\caption{Weight patterns of deep unfolding network when training in GAN model.}
%	\label{fig:gan_weight_15_11}
%\end{figure}

==> experiments3.tex <==
\section{Experiments}
\label{sec:exps}

We demonstrate the better decoding performance of our model in comparison with the original deep unfolding network and BP decoder on various codes.

\begin{figure*}[!t]
	\centering
	\begin{subfigure}[b]{0.41\linewidth}
		\includegraphics[width=\linewidth]{fig/bch_15_11}
		\caption{BCH(15,11)}
	\end{subfigure}
	\begin{subfigure}[b]{0.41\linewidth}
		\includegraphics[width=\linewidth]{fig/bch_63_45}
		\caption{BCH(63,45)}
	\end{subfigure}
	%\includegraphics[width=0.7\linewidth]{fig/bch_15_11}
	\caption{Performance of different decoders on BCH code.}
	\vspace{-0.15in}
	\label{fig:bch_fer}
\end{figure*}
\begin{figure*}[!t]
	\centering
	\begin{subfigure}[b]{0.41\linewidth}
		\includegraphics[width=\linewidth]{fig/rs_15_11}
		\caption{RS(15,11)}
	\end{subfigure}
	\begin{subfigure}[b]{0.41\linewidth}
		\includegraphics[width=\linewidth]{fig/rs_31_27}
		\caption{RS(31,27)}
	\end{subfigure}
	%\includegraphics[width=0.7\linewidth]{fig/bch_15_11}
	\caption{Performance of different decoders of Reed-Solomon codes (SSID is an effective belief propagation method for RS).}
	\vspace{-0.15in}
	\label{fig:rs_fer}
\end{figure*}
%\kwang{Can we use red, green, and blue? Also, how about using different line styles for different scheme in addition to different markers, which have already been applied, for b\&w print? These suggestion also can be applied to Fig. 4.}

\subsection{Setting}
We tested on both BCH codes BCH(15,11), BCH(63,45), and Reed-Solomon codes RS(15,11), RS(31,27), with an AWGN channel and various signal-to-noise (SNR) ratios.
For BCH codes, we use the neural offset min-sum deep unfolding model, FNOMS, as in \cite{nachmani2018deep} that unfolds 5 BP iterations and adds a discriminator with two fully connected layers, each of size 1024 with sigmoid activation function, and a single neuron output layer.
For Reed-Solomon codes, the decoder network, namely DeepSSID, unfolds the Stochastic Shifting Based Iterative Decoding (SSID) model\cite{zhang2020iterative}.
We applied the Adam optimizer with learning rate of 0.001 for both decoder and discriminator training and batch size 64.
10000 and 100000 codewords are randomly drawn for training and testing, respectively.

%\kwang{Compare with the classic results of BCH codes with BP decoding. Provide the number of iterations for decoding for all schemes.}
%\kwang{As commented in the previous section, use truncation for the sum-product algorithm rather than the min-sum algorithm for a fair comparison with \cite{nachmani2018deep}. In general, the sum-product algorithm outperforms the min-sum algorithm.}

\subsection{Results}

We compare our model, denoted by \method, with the original deep unfolding model and BP method with 100 iterations.
The results are demonstrated in Figure~\ref{fig:bch_fer} for BCH codes and Figure~\ref{fig:rs_fer} for Reed-Solomon codes.
In both cases, the results show that \method{} achieves improved decoding performance compared to both previous deep unfolding networks and BP.
The improvement is approximately 0.5dB consistently across all signal-to-noise ratios and different codes.

Notably, the improvement of \method{} for shorter block length as in BCH(15,11) and RS(15,11) is more significant than for longer block length as in BCH(63,45) and RS(31,27).
This is possibly due to the fixed number of layers in the decoder network and suggests larger block codes may need more layers or deeper networks to perform well.

%Weight patterns when training in GAN model:
%\begin{figure}[!h]
%	\centering
%	\includegraphics[width=0.5\linewidth]{fig/gan_weight_pattern.png}
%	\caption{Weight patterns of deep unfolding network when training in GAN model.}
%	\label{fig:gan_weight_15_11}
%\end{figure}


==> intro1.tex <==
\section{Introduction}

Deep unfolding \cite{hershey2014deep} combines the learning power of emerging deep neural networks (DNNs) with rigorous analytical understanding of model-based iterative algorithms in communications to address multiple challenges across various tasks, i.e., decoders for error correcting codes \cite{nachmani2018deep,lugosch2017neural,lugosch2018learning,zhang2020iterative}, symbol detection \cite{shlezinger2020deepsic,shlezinger2019viterbinet,samuel2019learning,he2018model}, channel precoding \cite{balatsoukas2019neural}. On one hand, deep unfolding removes assumptions of existing algorithms on channel condition and can deal with both linear and non-linear channels, while enjoying the optimality guarantees of well understood iterative algorithms thanks to having the same structure. On the other hand, deep unfolding can speed up the computation by reducing the number of iterations needed to achieve certain performance due to the impressive learnability of deep neural networks requiring only a few layers corresponding to a small number of iterations in existing iterative algorithms.

We propose to improve the performance of deep unfolding model by leveraging the same idea in  in the Generative Adversarial Networks (GANs) of having two models competing in a game and together improving their performances. In our case, we have the deep unfolding decoder learning to decode received noisy signal and we design a discriminator to distinguish between the decoded signal and valid codes. The goal of the decoder is both finding a sequence of symbols that is as close as possible to the transmitted one and fooling the discriminator to believe in that the generated sequence is a valid code. Hence, the decoder will be able to generate a valid code that is as close as possible to the transmitted code, boosting the probability of successful decoding. We illustrate our idea in Figure~\ref{fig:demo}. In the ideal case, the discriminator teaches the decoder to avoid invalid code regions and, thus, increases the probability of the decoder generating valid codes, including the correct codes with respect to the noisy received signal. Given that, error correcting codes has certain structure, the invalid region could be very large compared to valid region and, hence, the benefit of having this discriminator is significant.

\begin{figure}[!h]
	\centering
	\includegraphics[width=0.7\linewidth]{fig/demo.pdf}
	\caption{Benefit of having a discriminator to boost the probability of successful decoding.}
	\label{fig:demo}
\end{figure}

==> intro2.tex <==
\section{Introduction}

Deep unfolding \cite{hershey2014deep} combines the learning power of emerging deep neural networks (DNNs) with rigorous analytical understanding of model-based iterative algorithms in communications to address multiple challenges across various tasks, e.g., decoders for error correcting codes \cite{nachmani2018deep,lugosch2017neural,lugosch2018learning,zhang2020iterative}, symbol detection \cite{shlezinger2020deepsic,shlezinger2019viterbinet,samuel2019learning,he2018model}, and MIMO precoding \cite{balatsoukas2019neural}.
On the one hand, deep unfolding removes assumptions of existing algorithms on channel condition and can deal with both linear and nonlinear channels, while enjoying the optimality guarantees of well understood iterative algorithms thanks to having the same structure \cite{yedidia2001characterization,kuck2020belief}.
On the other hand, deep unfolding can speed up the computation by reducing the number of iterations needed to achieve certain performance due to the impressive learnability of deep neural networks, requiring only a few layers corresponding to a small number of iterations in existing iterative algorithms.

%\begin{figure}[!h]
%	\centering
%	\includegraphics[width=0.8\linewidth]{fig/demo.pdf}
%	\caption{Benefit of having a discriminator to boost the probability of successful decoding.}
%	\label{fig:demo}
%\end{figure}

We propose to improve the performance of deep unfolding models by leveraging the same idea used in Generative Adversarial Networks (GANs) of having two models competing in a game and together improving their performances.
In our case, we have the deep unfolding decoder learning to decode a received (noisy) signal and design a discriminator to distinguish between codewords and the decoded words.
The goal of the decoder is both recovering a sequence that is as close as possible to the transmitted codeword and fooling the discriminator to believe in that the decoded sequence is an actual codeword.
Hence, the decoder will be able to recover a codeword that is as similar as possible to the transmitted one, boosting the probability of successful decoding.
% We illustrate our idea in Figure~\ref{fig:demo}. 
In the ideal case, the discriminator teaches the decoder to avoid non-codeword regions; thus, it increases the probability of the decoder recovering codewords, including the correct codeword with respect to the noisy received signals.
Given that an error correcting code has certain structure, the non-codeword region could be very large compared to codeword region and, hence, the benefit of having this discriminator is significant.

Our game-theoretical model combining a deep unfolding network and a discriminator enjoys multiple advantageous properties.
We first prove that the optimal maximum likelihood (ML) decoder of a code along with a custom trained discriminator form a Nash equilibrium of our game model (Subsection~\ref{subsec:approach_ml}).
This establishes a strong connection between our model and the optimal ML decoder; if we train the model till convergence (equilibrium), it has a good chance of approaching the optimal ML decoder.
Furthermore, we show that a simple variant of our model also preserves all the fixed points of the original belief propagation (BP) decoder (Subsection~\ref{subsec:bp_fixed}).
These fixed points correspond to solutions of minimizing the Bethe free energy \cite{yedidia2003understanding}, which is important for inference tasks on factor graphs.
We experimentally verify that our model leads to improved decoding performance on various error correcting codes when compared with the original deep unfolding model and the BP algorithm (Section~\ref{sec:exps}).

%\kwang{This reasoning is not clear as yet. $2^k$ codewords of a block code of length $n$ forms a $k$-dimensional subspace of the vector space of all the $n$-tuple over the field $GF(2)$; thus, for most good error correcting codes, the codeword space is much smaller the space of any other sequences. However, this does not necessarily mean that the benefit of having the discriminator is significant, because the existing decoders (either NN-optimized decoders or classic decoders) also aim to classify received sequences into a transmitted codeword or not by inherently avoiding invalid codewords region. We are digging into a question, ''How and how effectively the discriminator can play a role suppressing the invalid codewords region compared to the existing decoders' capabilities?'' Can theory behind GAN provide us more detailed guidance in designing NN-optimized decoding algorithms beyond our current understanding above? If so, how?}



==> intro3.tex <==
\section{Introduction}
New data-intensive use cases (e.g., autonomous driving, high-precision industrial plants) demand high throughput and ultra-reliable and low latency communications for the fifth \cite{TS38.104} and subsequent generation networks. This demand requires iterative communication algorithms with a minimal number. However, little is theoretically known about optimal parameter tuning under strict iterative constraints and is usually established using heuristics via simulations or pessimistic bounds in practice \cite{Balatsoukas--Studer2019}.

%use cases and deployment requirements (e.g., eMBB and uRLLC in 5G NR) require information recovery with high throughput and/or very low latency for 5G \cite{TS38.104} and subsequent generation networks. This implies that iterative algorithms with a minimal number are desired. However, little is theoretically known about optimal parameter tuning under strict iterative constraints and is usually established using heuristics via simulations or pessimistic bounds in practice.

% Deep unfolding \cite{hershey2014deep} combines the learning power of emerging deep neural networks (DNNs) with rigorous analytical understanding of model-based iterative algorithms in communications to address multiple challenges across various tasks, e.g., decoders for error correcting codes \cite{nachmani2018deep,lugosch2017neural,lugosch2018learning,zhang2020iterative}, symbol detection \cite{shlezinger2020deepsic,shlezinger2019viterbinet,samuel2019learning,he2018model}, and MIMO precoding \cite{balatsoukas2019neural}.

Deep unfolding \cite{hershey2014deep} has been introduced as a promising approach to address these challenges across various tasks, e.g., decoders for error correcting codes \cite{nachmani2018deep,lugosch2017neural,lugosch2018learning,zhang2020iterative}, symbol detection \cite{shlezinger2020deepsic,shlezinger2019viterbinet,samuel2019learning,he2018model}, and MIMO precoding \cite{balatsoukas2019neural} by combining the learning power of emerging deep neural networks (DNNs) with rigorous analytical understanding of model-based  iterative algorithms in communications.
On the one hand, deep unfolding removes assumptions of existing algorithms on channel condition and can deal with both linear and nonlinear channels, while enjoying the optimality guarantees of well understood iterative algorithms thanks to having the same structure \cite{yedidia2001characterization,kuck2020belief}.
On the other hand, deep unfolding can speed up the computation by reducing the number of iterations needed to achieve certain performance due to the impressive learnability of deep neural networks, requiring only a few layers corresponding to a small number of iterations in existing iterative algorithms.

%\begin{figure}[!h]
%	\centering
%	\includegraphics[width=0.8\linewidth]{fig/demo.pdf}
%	\caption{Benefit of having a discriminator to boost the probability of successful decoding.}
%	\label{fig:demo}
%\end{figure}

We propose to improve the performance of deep unfolding models by leveraging the same idea used in Generative Adversarial Networks (GANs) of having two models competing in a game and together improving their performances.
In our case, we have the deep unfolding decoder learning to decode a received (noisy) signal and design a discriminator to distinguish between codewords and the decoded words.
The goal of the decoder is both recovering a sequence that is as close as possible to the transmitted codeword and fooling the discriminator to believe in that the decoded sequence is an actual codeword.
Hence, the decoder will be able to recover a codeword that is as similar as possible to the transmitted one, boosting the probability of successful decoding.
% We illustrate our idea in Figure~\ref{fig:demo}.
In the ideal case, the discriminator teaches the decoder to avoid non-codeword regions; thus, it increases the probability of the decoder recovering codewords, including the correct codeword with respect to the noisy received signals.
Given that an error correcting code has certain structure, the non-codeword region could be very large compared to codeword region and, hence, the benefit of having this discriminator is significant.

Our game-theoretical model combining a deep unfolding network and a discriminator enjoys multiple advantageous properties.
We first prove that the optimal maximum likelihood (ML) decoder of a code along with a custom trained discriminator form a Nash equilibrium of our game model (Subsection~\ref{subsec:approach_ml}).
This establishes a strong connection between our model and the optimal ML decoder; if we train the model till convergence (equilibrium), it has a good chance of approaching the optimal ML decoder.
Furthermore, we show that a simple variant of our model also preserves all the fixed points of the original belief propagation (BP) decoder (Subsection~\ref{subsec:bp_fixed}).
These fixed points correspond to solutions of minimizing the Bethe free energy \cite{yedidia2003understanding}, which is important for inference tasks on factor graphs.
We experimentally verify that our model leads to improved decoding performance on various error correcting codes when compared with the original deep unfolding model and the BP algorithm (Section~\ref{sec:exps}).


==> preliminary1.tex <==
\section{Preliminaries}

Here we summarize the message passing belief propagation Sum-Product and Min-Sum algorithms along with their deep unfolding neural network models. 

\subsection{Belief propagation (BP) algorithms}

The belief propagation (BP) decoder for a linear code with some parity check matrix can be constructed from the Tanner graph of the parity check matrix. The Tanner graph contains check and variable nodes arranged as a bipartite graph, and edges between check and variable nodes, which represent messages passing between those nodes. Denote by $N$, the code block length (i.e., the number of variable nodes in the Tanner graph). A simple example is given in Figure~\ref{fig:bp}.(a) with $N = 3$ variable nodes. Each iteration in the BP decoder corresponds to one round of messaging passing between variable and check nodes. 
\begin{figure}[!h]
	\centering
	\includegraphics[width=0.7\linewidth]{fig/bp_illustrate.pdf}
	\vspace{-0.1in}
	\caption{Tanner graph and Trellis representation of a BP decoder.}
	\label{fig:bp}
\end{figure}
In iteration $i$, on the edge $e = (v,c)$ variable node $v$ passes the following message $x_{i, (v,c)}$ to the check node $c$:
\begin{align}
	x_{i, e = (v,c)} = l_v + \sum_{e' = (c',v), c' \neq c} x_{i-1, e'},
\end{align}
where $l_v$ is the log-likelihood ratio of the channel output corresponding to the $v$th codebit $C_v$:
\begin{align}
	l_v = \log\frac{\Pr(C_v = 1 | y_v)}{\Pr(C_v = 0 | y_v)}.
\end{align}

In the Sum-Product algorithm, the message $x_{i, (c,v)}$ from check node $c$ to variable node $v$ in iteration $i$ is computed as follows:
\begin{align}
	x_{i, e = (c,v)} = 2 \tanh^{-1}\left( \prod_{e' = (v',c), v' \neq v} \tanh \frac{x_{i,e'}}{2} \right).
\end{align}
However, this computation involves repeated multiplications and hyperbolic functions, which may lead to numerical problems in actual implementation. Thus the Min-Sum algorithm uses a ``min-sum'' approximation of the above message as follows:
\begin{align}
	x_{i, e = (c,v)} = \min_{e' = (v',c), v' \neq v} |x_{i,e'}| \prod_{e' = (v',c), v' \neq v} \sign(x_{i,e'}).
\end{align}

Suppose that BP decoder runs $L$ iterations, the final $v$th output is given by:
\begin{align}
	\label{eq:output}
	o_v = l_v + \sum_{e' = (c',v)} x_{L,e'}.
\end{align}

\subsection{Unfolding BP models}

The BP decoder has an equivalent Trellis representation that motivates the unfolding neural network architecture. An simple example is provided in Figure~\ref{fig:bp}.(b). Each BP iteration $i$ unfolds into 2 hidden layers $2\times i-1$ and $2\times i$ corresponding to 2 passes of message from variable to check nodes and, vice versus, from check to variable nodes. The number of nodes in each hidden layer is the same as the number of edges in the Tanner graph and, respectively, each node computes the message sent through each edge. Thus, there are $2\times L$ hidden layers in this Trellis representation in addition to an input and output layer. The input takes log-likelihood ratios of channel outputs and the output computes Eq.~\ref{eq:output}.

The unfolding neural network model share the exact same architecture as the Trellis representation and add trainable weights to the edges. Thus, in odd layer $i$, the computation at node $i, e = (v,c)$ perform the following operation:
\begin{align}
	x_{i, e = (v,c)} = \tanh \left(\frac{1}{2}\left (w_{i,v}l_v + \sum_{e' = (c',v), c' \neq c} w_{i,e,e'}x_{i-1, e'} \right) \right).
\end{align}
In even layer $i$, the computation at node $i, e = (v,c)$ is as follows:
\begin{align}
	x_{i, e = (c,v)} = 2 \tanh^{-1}\left( \prod_{e' = (v',c), v' \neq v} x_{i-1,e'} \right).
\end{align}
Node at the output layer performs:
\begin{align}
	o_v = \sigma \left(w_{2L + 1,v}l_v + \sum_{e' = (c',v)} w_{2L+1,v,e'} x_{2L,e'} \right ).
\end{align}

==> preliminary2.tex <==
\section{Preliminaries}

In this section, we review the well known belief propagation (BP) method for error correcting codes and the deep neural network model that is constructed by deep unfolding this BP method.
Here we summarize the message passing belief propagation Sum-Product and Min-Sum algorithms along with their deep unfolding neural network models.

\textbf{Channel noise model.} We consider a common channel model where additive random noise follows a Gaussian distribution with mean $0$ and variance $\sigma^2$, i.e., $N(0, \sigma^2)$.
We follow the common assumption that transmitted codewords are uniformly selected at random from the set of all codewords.

\subsection{Belief propagation (BP) algorithms}

Given a linear error correcting code $\mathbb{C}$ of block-length $n$, characterized by a parity check matrix $\mathbf{H}$ of size $n \times (n-k)$, every codeword $\x \in \mathbb{C}$ satisfies $\mathbf{H}^T \x = \0$, where $\mathbf{H}^T$ denotes the transpose of $\mathbf{H}$ and $\0$ the vector of $n-k$ zeros.

The BP decoder for a linear code can be constructed from the Tanner graph of the parity check matrix.
The Tanner graph contains $n-k$ check nodes and $n$ variable nodes arranged as a bipartite graph with edges between check and variable nodes, which represent messages passing between these nodes.
If $\mathbf{H}_{vc} = 1$, there is an edge between variable node $v$ and check node $c$.
A simple example is given in Figure~\ref{fig:bp}(a) with $n = 3$ variable nodes and $(n-k) = 2$ check nodes.
The BP decoder consists of multiple iterations.
Each iteration corresponds to one round of messaging passing between variable and check nodes. 
\begin{figure}[!h]
	\centering
	\vspace{-0.1in}
	\includegraphics[width=\linewidth]{fig/bp_illustrate2.pdf}
	\caption{Tanner graph of a code and BP unfolding architecture.}
	\label{fig:bp}
\end{figure}
In iteration $i$, on edge $e = (v,c)$, the message $x_{i, (v,c)}$ passed from variable node $v$ to the check node $c$ is given by
\begin{align}
	\label{eq:m_vc_bp}
	x_{i, e = (v,c)} = l_v + \sum_{e' = (c',v), c' \neq c} x_{i-1, e'},
\end{align}
where $l_v$ is the log-likelihood ratio of the channel output corresponding to the $v$th codeword bit $C_v$.
Given random Gaussian noise, the log-likelihood ratio $l_v$ is
\begin{align}
	l_v = \log\frac{\Pr(C_v = 1 | y_v)}{\Pr(C_v = 0 | y_v)}.
\end{align}

In the Sum-Product algorithm, the message $x_{i, (c,v)}$ from check node $c$ to variable node $v$ in iteration $i$ is computed as
\begin{align}
	\label{eq:m_cv_bp}
	x_{i, e = (c,v)} = 2 \tanh^{-1}\left( \prod_{e' = (v',c), v' \neq v} \tanh \frac{x_{i,e'}}{2} \right).
\end{align}
For numerical stability, the messages going into a node in both Eq.~(\ref{eq:m_vc_bp}) and Eq.~(\ref{eq:m_cv_bp}) are normalized at every iteration and all the messages are also truncated within a fixed range.

Note that the computation in Eq.~(\ref{eq:m_cv_bp}) involves repeated multiplications and hyperbolic functions, which may lead to heavy computation and numerical problems in actual implementations.
Even with truncation of message values within a certain range, e.g., commonly $[-10, 10]$, we still observe numerical problems when running Sum-Product algorithm.

%\kwang{Truncate the messages from variable nodes to a check node into a specific range (e.g., -15.0 $\sim$ 15.0). It sets the size of the input messages in the check nodes to a level that does not cause numerical problems.}

The Min-Sum algorithm uses a ``min-sum'' approximation of the above message as follows:
\begin{align}
	x_{i, e = (c,v)} = \min_{e' = (v',c), v' \neq v} |x_{i,e'}| \prod_{e' = (v',c), v' \neq v} \sign(x_{i,e'}).
\end{align}

Suppose the BP decoder runs $L$ iterations. Then the $v$th output after final iteration is given by
\begin{align}
	\label{eq:output}
	o_v = l_v + \sum_{e' = (c',v)} x_{L,e'}.
\end{align}

\subsection{Unfolding BP models}

The BP decoder has an equivalent Trellis representation that motivates the unfolding neural network architecture.
A simple example is provided in Figure~\ref{fig:bp}(b).
Each BP iteration $i$ unfolds into 2 hidden layers, $2\times i-1$ and $2\times i$, corresponding to two passes of messages from variable to check nodes and from check to variable nodes.
The number of nodes in each hidden layer is the same as the number of edges in the Tanner graph and, respectively, each node computes the message sent through each edge.
Thus, there are $2\times L$ hidden layers in this Trellis representation in addition to an input and output layer.
The input takes log-likelihood ratios of channel received signals and the output computes Eq.~\ref{eq:output}.

The unfolding neural network model shares the same architecture as the Trellis representation and adds trainable weights to the edges.
In other words, in odd layer $i$, the computation at node $i, e = (v,c)$, performs the following operation (activation function):
\begin{align}
	\label{eq:m_vc}
	x_{i, e = (v,c)} = w_{i,v}l_v + \sum_{e' = (c',v), c' \neq c} w_{i,e,e'}x_{i-1, e'}.
\end{align}
Note that trainable weights $w_{i,v}$ and $w_{i,e,e'}$ are introduced in the computation.
These weights can be trained and address various challenging obstacles with the BP method: 1) reduce the large number of iterations needed in BP, leading to more efficiency; 2) improve decoding performance and possibly approach optimal ML criterion, thanks to the ability to possibly minimize the effects of short cycles known to cause difficulties for BP decoders.

In even layer $i$, the computation at node $i, e = (v,c)$ is similar to that in the regular BP algorithm:
\begin{align}
	\label{eq:m_cv}
	x_{i, e = (c,v)} = 2 \tanh^{-1}\left( \prod_{e' = (v',c), v' \neq v} \tanh \frac{x_{i-1,e'}}{2} \right).
\end{align}
For numerical stability, we also apply normalization and truncation of messages after every layer.

Nodes at the output layer perform
\begin{align}
	\label{eq:o_v}
	o_v = \sigma \left(w_{2L + 1,v}l_v + \sum_{e' = (c',v)} w_{2L+1,v,e'} x_{2L,e'} \right ),
\end{align}
where $\sigma(.)$ is the sigmoid function to obtain probability from the log-likelihood ratio representation.
Note that trainable weights $w_{2L + 1,v}$ and $w_{2L+1,v,e'}$ are also introduced here.

==> preliminary3.tex <==
\section{Preliminaries}

In this section, we review the well known belief propagation (BP) method for error correcting codes and the deep neural network model that is constructed by deep unfolding this BP method.
Here we summarize the message passing belief propagation sum-product and min-sum algorithms along with their deep unfolding neural network models.

We consider the discrete-time additive white Gaussian noise (AWGN) channel model. In transmission time $i \in [1:n]$, the channel output is $Y_i = gX_i + Z_i$. where $g$ is the channel gain, $X_i \in \{ \pm 1\}$, $\{ Z_i \}$ is a AWGN ($\sigma^2$) process, independent of the channel input $X^n = x^n(m)$, $m \in [1:2^{k}]$, and $k$ is the message length.

% \textbf{Channel noise model.} We consider a common channel model where additive random noise follows a Gaussian distribution with mean $0$ and variance $\sigma^2$, i.e., $N(0, \sigma^2)$.
% We follow the common assumption that transmitted codewords are uniformly selected at random from the set of all codewords.

\subsection{Belief Propagation (BP) Algorithms}

Given a linear error correcting code $C$ of block-length $n$, characterized by a parity check matrix $H$ of size $n \times (n-k)$, every codeword $x \in C$ satisfies $H^T x = \0$, where $H^T$ denotes the transpose of $H$ and $0$ the vector of $n-k$ zeros.

% Given a linear error correcting code $\mathbb{C}$ of block-length $n$, characterized by a parity check matrix $\mathbf{H}$ of size $n \times (n-k)$, every codeword $\x \in \mathbb{C}$ satisfies $\mathbf{H}^T \x = \0$, where $\mathbf{H}^T$ denotes the transpose of $\mathbf{H}$ and $\0$ the vector of $n-k$ zeros.

The BP decoder for a linear code can be constructed from the Tanner graph of the parity check matrix.
The Tanner graph contains $n-k$ check nodes and $n$ variable nodes arranged as a bipartite graph with edges between check and variable nodes, which represent messages passing between these nodes.
If $H_{vc} = 1$, there is an edge between variable node $v$ and check node $c$.
% If $\mathbf{H}_{vc} = 1$, there is an edge between variable node $v$ and check node $c$.
A simple example is given in Figure~\ref{fig:bp}(a) with $n = 3$ variable nodes and $(n-k) = 2$ check nodes.
The BP decoder consists of multiple iterations.
Each iteration corresponds to one round of messaging passing between variable and check nodes.
\begin{figure}[!t]
	\centering
	\vspace{-0.1in}
	\includegraphics[width=\linewidth]{fig/bp_illustrate2.pdf}
	\caption{Tanner graph of a code and BP unfolding architecture.}
	\vspace{-0.15in}
	\label{fig:bp}
\end{figure}
In iteration $i$, on edge $e = (v,c)$, the message $x_{i, (v,c)}$ passed from variable node $v$ to the check node $c$ is given by
\begin{align}
	\label{eq:m_vc_bp}
	x_{i, e = (v,c)} = l_v + \sum_{e' = (c',v), c' \neq c} x_{i-1, e'},
\end{align}
where $l_v$ is the log-likelihood ratio of the channel output corresponding to the $v$th codeword bit $C_v$, i.e.,
% Given random Gaussian noise,
%The log-likelihood ratio $l_v$ is
\begin{align}
	l_v = \log\frac{\Pr(C_v = 1 | y_v)}{\Pr(C_v = 0 | y_v)}. \nonumber
\end{align}

In the sum-product algorithm, the message $x_{i, (c,v)}$ from check node $c$ to variable node $v$ in iteration $i$ is computed as
\begin{align}
	\label{eq:m_cv_bp}
	x_{i, e = (c,v)} = 2 \tanh^{-1}\Big( \prod_{e' = (v',c), v' \neq v} \tanh \frac{x_{i,e'}}{2} \Big).
\end{align}
For numerical stability, the messages going into a node in both Eq.~(\ref{eq:m_vc_bp}) and Eq.~(\ref{eq:m_cv_bp}) are normalized at every iteration and all the messages are also truncated within a fixed range.

Note that the computation in Eq.~(\ref{eq:m_cv_bp}) involves repeated multiplications and hyperbolic functions, which may lead to numerical problems in actual implementations. Even with truncation of message values within a certain range, e.g., commonly $[-10, 10]$, we still observe numerical problems when running the sum-product algorithm.
% Thus, we consider the Min-Sum algorithm in this paper.

% Note that the computation in Eq.~(\ref{eq:m_cv_bp}) involves repeated multiplications and hyperbolic functions, which may lead to heavy computation and numerical problems in actual implementations.
% Even with truncation of message values within a certain range, e.g., commonly $[-10, 10]$, we still observe numerical problems when running Sum-Product algorithm.

%\kwang{Truncate the messages from variable nodes to a check node into a specific range (e.g., -15.0 $\sim$ 15.0). It sets the size of the input messages in the check nodes to a level that does not cause numerical problems.}

The min-sum algorithm uses a ``min-sum'' approximation of the above message as follows:
\begin{align}
	x_{i, e = (c,v)} = \min_{e' = (v',c), v' \neq v} |x_{i,e'}| \prod_{e' = (v',c), v' \neq v} \sign(x_{i,e'}). \nonumber
\end{align}
Suppose the BP decoder runs $L$ iterations. Then the $v$th output after final iteration is given by
\begin{align}
	\label{eq:output}
	o_v = l_v + \sum_{e' = (c',v)} x_{L,e'}.
\end{align}

\subsection{Unfolding BP Models}
The BP decoder has an equivalent Trellis representation that motivates the unfolding neural network architecture.
A simple example is provided in Figure~\ref{fig:bp}(b).
Each BP iteration $i$ unfolds into 2 hidden layers, $2\times i-1$ and $2\times i$, corresponding to two passes of messages from variable to check nodes and from check to variable nodes.
The number of nodes in each hidden layer is the same as the number of edges in the Tanner graph and, respectively, each node computes the message sent through each edge.
Thus, there are $2\times L$ hidden layers in this Trellis representation in addition to an input and output layer.
The input takes log-likelihood ratios of channel received signals and the output computes Eq.~\ref{eq:output}.

The unfolding neural network model shares the same architecture as the Trellis representation and adds trainable weights to the edges.
In other words, in odd layer $i$, the computation at node $i, e = (v,c)$, performs the following operation (activation function):
\begin{align}
	\label{eq:m_vc}
	x_{i, e = (v,c)} = w_{i,v}l_v + \sum_{e' = (c',v), c' \neq c} w_{i,e,e'}x_{i-1, e'}.
\end{align}
Note that trainable weights $w_{i,v}$ and $w_{i,e,e'}$ are introduced in the computation.
These weights can be trained and address various challenging obstacles with the BP method: 1) reduce the large number of iterations needed in BP, leading to more efficiency; 2) improve decoding performance and possibly approach optimal ML criterion, thanks to the ability to possibly minimize the effects of short cycles known to cause difficulties for BP decoders.

In even layer $i$, the computation at node $i, e = (v,c)$ is similar to that in the regular BP algorithm:
\begin{align}
	\label{eq:m_cv}
	x_{i, e = (c,v)} = 2 \tanh^{-1}\Big( \prod_{e' = (v',c), v' \neq v} \tanh \frac{x_{i-1,e'}}{2} \Big).
\end{align}
For numerical stability, we also apply normalization and truncation of messages after every layer.

Nodes at the output layer perform
\begin{align}
	\label{eq:o_v}
	o_v = \sigma \Big(w_{2L + 1,v}l_v + \sum_{e' = (c',v)} w_{2L+1,v,e'} x_{2L,e'} \Big),
\end{align}
where $\sigma(.)$ is the sigmoid function to obtain probability from the log-likelihood ratio representation.
Note that trainable weights $w_{2L + 1,v}$ and $w_{2L+1,v,e'}$ are also introduced here.

